LIST: Learning to Index Spatio-Textual Data for Embedding based Spatial Keyword Queries

With the proliferation of spatio-textual data, Top-k KNN spatial keyword queries (TkQs), which return a list of objects based on a ranking function that considers both spatial and textual relevance, have found many real-life applications. To efficiently handle TkQs, many indexes have been developed, but the effectiveness of TkQ is limited. To improve effectiveness, several deep learning models have recently been proposed, but they suffer severe efficiency issues and there are no efficient indexes specifically designed to accelerate the top-k search process for these deep learning models. To tackle these issues, we consider embedding based spatial keyword queries, which capture the semantic meaning of query keywords and object descriptions in two separate embeddings to evaluate textual relevance. Although various models can be used to generate these embeddings, no indexes have been specifically designed for such queries. To fill this gap, we propose LIST, a novel machine learning based Approximate Nearest Neighbor Search index that Learns to Index the Spatio-Textual data. LIST utilizes a new learning-to-cluster technique to group relevant queries and objects together while separating irrelevant queries and objects. There are two key challenges in building an effective and efficient index, i.e., the absence of high-quality labels and the unbalanced clustering results. We develop a novel pseudo-label generation technique to address the two challenges. Additionally, we introduce a learning based spatial relevance model that can integrates with various text relevance models to form a lightweight yet effective relevance for reranking objects retrieved by LIST.

==> abstract.tex <==
\begin{abstract}
With the proliferation of spatio-textual data, Top-k KNN spatial keyword queries (\tkskqs), which return a list of objects based on a ranking function that considers both spatial and textual relevance, have found many real-life applications. %Existing geo-textual indexes for 
To efficiently handle \tkskqs, many indexes have been developed, but the effectiveness of \tkskq is limited. %commonly 
% uses traditional information} retrieval models like BM25 to compute text relevance and exploit a simple linear function to compute spatial relevance, which leads to limited effectiveness. 
To improve effectiveness, several deep learning models have recently been proposed, but they suffer severe efficiency issues and there are no efficient indexes specifically designed to accelerate the top-k search process for these deep learning models.

% To tackle these issues, we propose a novel technique, which \underline{L}earns to \underline{I}ndex the \underline{S}patio-\underline{T}extual data for answering  embedding based spatial keyword queries (called \Framework). \Framework is featured with two novel components. Firstly, we propose a lightweight and effective relevance model that is capable of learning both spatial and textual relevance. Secondly, we introduce a novel machine learning based Approximate Nearest Neighbor Search (ANNS) index to accelerate the top-k search process of the proposed relevance model, which utilizes a new learning-to-cluster technique to group relevant queries and objects together while separating irrelevant queries and objects. There exist two key challenges in building an effective and efficient index, i.e., the absence of high-quality labels and the unbalanced clustering results. We develop a novel pseudo-label generation technique to address the two challenges. Experimental results show that \Framework significantly outperforms state-of-the-art methods on effectiveness, with improvements up to 19.21\% and 12.79\% in terms of NDCG@1 and Recall@10, and is three orders of magnitude faster than the most effective baseline.  


To tackle these issues, \revision{we consider embedding based spatial keyword queries, which capture the semantic meaning of query keywords and object descriptions in two separate embeddings to evaluate textual relevance. Although various 
%text 
models can be used to generate these embeddings, no indexes have been specifically designed for such queries. To fill this gap, we propose \Framework, a novel machine learning based Approximate Nearest Neighbor Search index that \underline{L}earns to \underline{I}ndex the \underline{S}patio-\underline{T}extual data. %for answering embedding based spatial keyword queries (called \Framework). 
\Framework utilizes a new learning-to-cluster technique to group relevant queries and objects together while separating irrelevant queries and objects. There are two key challenges in building an effective and efficient index, i.e., the absence of high-quality labels and the unbalanced clustering results. We develop a novel pseudo-label generation technique to address the two challenges. Additionally, we introduce a learning based spatial relevance model that can integrates with various text relevance models to form a lightweight yet effective relevance for reranking objects retrieved by \Framework. Experimental results show that (1) our lightweight embedding based relevance model significantly outperforms  state-of-the-art relevance models; (2) \Framework outperforms state-of-the-art indexes, providing a better trade-off between effectiveness and efficiency.} 



\end{abstract}



==> conclusion.tex <==
\section{Conclusions and Future Work}
In this paper, \revision{we propose a novel index \Framework for embedding based spatial keyword queries. 
%and the relevance models tailored for such queries.
} We conduct extensive experiments to show the effectiveness and efficiency of \Framework over the state-of-the-art index baselines. This work opens up a promising research direction of designing novel ANNS indexes for accelerating the search for embedding based spatial keyword queries. One interesting future direction is integrating our index with product quantization techniques to further expedite the search process. Another potential direction is to extend our proposed index to vector databases for dense vectors without spatial information. 

==> exp.tex <==
% \vspace*{-0.5em}
\section{Experiments}
% \vspace*{-0.5em}

\label{sec:exp}
In this section, we evaluate the effectiveness and efficiency of our proposed solution for answering \tkskqs by comparing it with state-of-the-art methods on three real-world datasets. We aim to answer the following research questions: 

% How do the two major components perform, i.e., the proposed relevance model and the index? 


\begin{itemize}[leftmargin=*,topsep=0pt]
    % \item \textbf{RQ1:} Does our proposed retriever \Framework and our proposed relevance model outperform previous state-of-the-art methods in terms of effectiveness?
    % \item \textbf{RQ2:} How well does the efficiency of our proposed retriever \Framework compare with state-of-the-art methods? 
    \item \textbf{RQ1:} \revision{Does our relevance model outperform existing relevance models in terms of effectiveness?}
    \item \textbf{RQ2:} \revision{Does our proposed ANNS index achieve a better effectiveness-efficiency trade-off compared to existing indexes?}
    \item \textbf{RQ3:} \revision{Can our proposed ANNS index be applied to other relevance models designed for embedding based spatial keyword queries?}    
    \item \textbf{RQ4:} How does \Framework scale with the size of dataset?    
    \item \textbf{RQ4:} What are the impacts of our proposed index and different modules in the proposed \Framework? 

    
    % \item  \textbf{RQ5:} How does training data size affect the performance of our proposed retriever \Framework and our proposed relevance model?
    
    %How does the size of training data affect our proposed retriever \Framework and proposed relevance model?
    
\end{itemize}





\begin{table}[!t]
    \centering
    \caption{Datasets Statistics.}
    % \vspace*{-0.5em}
    \label{tab:dataset}
    \renewcommand{\arraystretch}{1.2} % 控制行高
    \setlength{\arrayrulewidth}{0.5pt}
    % \small
    \begin{tabularx}{0.5\textwidth}{>{\centering}m{3.6cm}*{2}{X}m{1.5cm}}
    \toprule[1pt]
    \multirow{2}{*}{} & Beijing & Shanghai & Geo-Glue\\
    \midrule[1pt]
    Number of Pois & 122,420 & 116,859 & 2,849,754\\
    Number of Queries & 168,998 & 127,183 & 90,000\\
    Number of Records & 233,343 & 182,634 & 90,000\\
    \midrule
    Number of Train Queries & 136,890 & 103,019 & 50,000 \\
    Number of Val Queries& 15,209 & 11,446 & 20,000 \\
    Number of Test Queries& 16,899 & 12,718 & 20,000 \\
    \midrule
    Number of Train Records & 189,027 & 148,017 & 50,000 \\
    Number of Val Records& 21,034 & 16,492 & 20,000 \\
    Number of Test Records& 23,282 & 18,125 & 20,000\\    
    \bottomrule[1pt]
    \end{tabularx}
    % \vspace*{-2em}
\end{table}

% \vspace*{-1em}
\subsection{Experimental Setup}
\label{sec:exp-setup}
\noindent\textbf{Datasets.} To evaluate the effectiveness and efficiency of our proposed retriever \Framework, we utilize three benchmark datasets: Beijing, Shanghai, and Geo-Glue. Among them, the Beijing and Shanghai datasets~\cite{liu2023effectiveness} are provided 
%by Meituan, 
a Chinese retail services platform. Users submit a query through the platform, which consists of a query location and a set of keywords. Subsequently, the Points of Interest (POIs) that users clicked on are recorded in the query log, and is considered as a ground-truth. Note that the click-through data recorded in the search log may be the only feasible way to get a large scale of ground truth data for spatial keyword queries~\cite{liu2023effectiveness}. The explicit feedback such as ratings is very challenging to collect~\cite{DBLP:conf/www/HeLZNHC17}. Note that using query logs is also the popular way of generating ground truth in the Information Retrieval literature~\cite{DBLP:conf/www/HeLZNHC17,DBLP:conf/cikm/HuangHGDAH13,DBLP:conf/www/YaoTCYXD021,DBLP:conf/kdd/Joachims02}. Therefore, following the previous work~\cite{liu2023effectiveness}, we utilize the two datasets to evaluate our proposed solution \Framework and treat the clicked POIs as ground truth relevant objects to the corresponding queries. In the Geo-Glue dataset~\cite{li2023geoglue,DBLP:conf/sigir/DingCXHLZX23}.
%is released by DAMO Academic. The 
the POIs  are crawled from OpenStreetMap\footnote{https://www.openstreetmap.org/}, and the queries and the corresponding ground truth POIs are manually generated by domain experts. Notably, in the released Geo-Glue dataset, the coordinates of objects and queries are modified due to privacy considerations, which results in many objects with identical geo-locations.



% We utilize three benchmark datasets: Beijing, Shanghai, and Geo-Glue. The Beijing and Shanghai datasets~\cite{liu2023effectiveness} are provided by Meituan, a Chinese retail services platform. Users submit queries consisting of location and keywords. Following previous work~\cite{liu2023effectiveness}, the clicked Points of Interest (POIs) recorded in the query log are regarded as the ground truth answers to these queries. %, which are presented as records in Table~\ref{tab:dataset}.
%According to \cite{liu2023effectiveness}, this approach may be the only feasible way to get a large scale of ground truth data. 
%Note that the click-through data recorded in the search log is widely used as ground-truth for information retrieval evaluation as explicit feedback such as ratings is challenging to collect and implicit feedback such as click-through data can be tracked automatically and is thus much easier to collect for content providers
% {\color{red} Note that the click-through data recorded in the search log may be the only feasible way to get a large scale of ground truth data as explicit feedback such as ratings is challenging to collect and implicit feedback such as click-through data can be tracked automatically~\cite{liu2023effectiveness, DBLP:conf/www/HeLZNHC17}. }

%Thus we follow previous work~\cite{liu2023effectiveness}, and generate ground truth using query logs, i.e., when users click a POI, it is considered as a ground truth for the query.
% thus scarce
%, while manual annotations are expensive.
%These search records are collected in a short period from Beijing and Shanghai respectively. 
% Both datasets are anonymized to protect user privacy and more details can be found here~\cite{liu2023effectiveness}. The Geo-Glue dataset~\cite{li2023geoglue,DBLP:conf/sigir/DingCXHLZX23} is released by DAMO Academic.
%, which is the largest open dataset available. 
% The POIs in the dataset are crawled from OpenStreetMap\footnote{https://www.openstreetmap.org/}, and the queries and the corresponding ground truth POIs are manually generated by domain experts. Notably, in the released Geo-Glue dataset, the coordinates of objects and queries are modified due to privacy considerations, which results in many objects with identical geo-locations.

%Note that, 

The release of query log datasets from the industry is highly restricted. {As a result, to the best of our knowledge, there are no other public datasets that contain ground-truth query results or query logs, except for the three datasets used in our experiments.} To investigate the scalability of the proposed framework, we conduct a scalability study to show \Framework's efficiency on larger datasets, where the Geo-Glue dataset is augmented with more crawled POIs from OpenStreetMap (as to be shown in Section~\ref{sec:exp-scalibility})









\begin{table}[!t]
    \centering
    \caption{\revision{Hyperparameter settings on three datasets.}}
    % \vspace*{-0.5em}
    \label{tab:hyper}
    \renewcommand{\arraystretch}{1.2} % 控制行高
    \setlength{\arrayrulewidth}{0.5pt}
    \small
    \begin{tabularx}{0.5\textwidth}{>{\centering}m{3.6cm}*{2}{X}m{1.5cm}}
    \toprule[1pt]
    Hyperparameters & Beijing & Shanghai & Geo-Glue\\
    \midrule[1pt]
    spatial footstep $t$ & 1000 & 1000 & 1000 \\
    pseudo-label's $\text{neg}_\text{start}$ & 50,000 & 60,000 & 180,000\\
    pseudo-label's $\text{neg}_\text{end}$ & 55,000 & 65,000 & 181,000\\
    number of cluster $c$ & 20 & 20  & 300 \\  
    \bottomrule[1pt]
    \end{tabularx}
    % \vspace*{-2em}
\end{table}

% \begin{table}[tpb!]
% \caption{Hyperparameter settings on three datasets.}
% \centering
% \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Datasets} & \textbf{Attention} & \textbf{Hidden} & \textbf{Layers in JK} & \textbf{Num Layers} & \textbf{Activation} \\ \hline
% Beijing   & Recursive & 512  & / & 4 & Leaky ReLU (a=0.2)  \\ \hline
% Shanghai & JK & 1280  & 4 & 6 & Sigmoid \\ \hline
% Geo-Glue & JK  & 512  & 4 & 4 & Leaky ReLU (a=0.2) \\ \hline
% \end{tabular}}
% \label{table:parameter}
% \end{table}

% {\color{red} Additionally, our techniques introduce nearly no extra space consumption. The only extra space consumption is brought by our proposed relevance model \Framework-R and the learned index model, which is ignorable compared with the huge $d$-dimensional database of size $n$. Thus, we do not report the memory consumption in the experiment.}

%\textit{Notably, in the released Geo-Glue dataset, the coordinates of objects and queries are modified due to privacy considerations, which results in many objects with identical geo-locations.}

%Note that, due to privacy considerations, the release of query log datasets from the industry is restricted. \textit{As a result, to our knowledge, no other datasets containing ground-truth query results have been released, except for the three datasets used in our experiment. To investigate the scalability of the proposed framework, we conduct a scalability study to show \Framework's efficiency on larger datasets, where the Geo-Glue dataset is augmented with more crawled POIs (shown in Section~\ref{sec:exp-scalibility})}

%To our knowledge, no other datasets containing ground-truth query results have been released, hence we conduct experiments on the three datasets. To investigate the scalability of the proposed framework, we augment the Geo-Glue dataset with more crawled POIs (shown in Section~\ref{sec:exp-scalibility}).






\noindent\textbf{Dataset Split.} The statistics of datasets are stated in Table~\ref{tab:dataset}, where each record represents a single ground-truth label between an object and a query, and each query may have multiple ground-truth objects. %records denote the ground-truth denote the ground-truth records between queries and objects. 
For the Beijing and Shanghai datasets, to ensure a fair comparison, we follow the previous split strategy~\cite{liu2023effectiveness}, where 90\% of queries and their corresponding ground-truth records are used as the training set and the remaining queries as the test set. From the training set, we randomly choose 10\% data as the validation set to tune hyperparameters. For the Geo-Glue dataset~\cite{DBLP:conf/sigir/DingCXHLZX23}, we follow the provided splits for training, validation, and test data.
\begin{table*}[t]
% \vspace*{-1em}
    \centering
    \caption{Comparison of relevance models across three datasets by brute-force search.}
    % \vspace*{-0.5em}
    \label{tab:relevance_model}
    % \small
    \renewcommand{\arraystretch}{1.5} % 控制行高
    \setlength{\arrayrulewidth}{0.5pt}
    \begin{tabularx}{1\textwidth}{>{\centering}m{2cm}*{4}{X}*{4}{X}*{4}{X}}
        \toprule[1pt]
        \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Beijing}} & \multicolumn{4}{c} {\textbf{Shanghai}} & \multicolumn{4}{c} {\textbf{Geo-Glue}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
        & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}}  &
        \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
        \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} \\
        \midrule[1pt]
        % BM25 & 0.3875 & 0.3259 & 0.2113 & 0.1601 & 0.4044 & 0.3225 & 0.1900 & 0.1217 & 0.5374& 0.4987 &0.3879 & 0.3108\\
        TkQ  & 0.5740 & 0.5283 & 0.4111 & 0.3302 & {0.6746} & 0.6380 & 0.5044 & 0.4009 & 0.5423 & \underline{0.5023} & \underline{0.3847} & 0.3051 \\
        % TkQ  & 0.4683 & 0.4020 & 0.2618 & 0.1921 & {0.5465} & 0.4520 & 0.2674 & 0.1727 & 0.5423 & 0.5023 & 0.3847 & 0.3051 \\

        PALM & 0.3514 & 0.3098 & 0.2077 & 0.1343 & 0.4617 & 0.4023 & 0.2065 & 0.1223 &  N/A & N/A &  N/A & N/A   \\        

        DrW & \underline{0.6968} & \underline{0.6316} & \underline{0.4814} & \underline{0.3791} & \underline{0.7689} & \underline{0.7159} & \underline{0.5394} & \underline{0.4114} & N/A & N/A &  N/A & N/A \\
        
        % DrW & {0.6968} & {0.6316} & {0.4814} & {0.3791} & {0.7689} & {0.7159} & {0.5394} & {0.4114} & N/A & N/A &  N/A & N/A \\
   
        % DPR & 0.5078 & 0.4269 & 0.2892 & 0.2209 & 0.5143 & 0.4161 & 0.2505 & 0.1721 & 0.7626 & 0.7249 & 0.6014  & 0.5079 \\
        % % DPR$_D$ & 0.6807 & 0.6150 & 0.4576 & 0.3690 & 0.7579 & 0.7042  & 0.5358 & \underline{0.4347} & \underline{0.7963} & \underline{0.7565} & \underline{0.6211} & 0.5202 \\

        % DPR$_D$ & \underline{0.7555} & \underline{0.6845} & \underline{0.5181} & \underline{0.4215} & \underline{0.7986} & \underline{0.7494}  & \underline{0.5769} & \underline{0.4568} & \underline{0.7963} & \underline{0.7565} & \underline{0.6211} & 0.5202 \\
        
        MGeo& N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & \underline{0.7049} & N/A & N/A  & \underline{0.5270} \\ 
        \midrule
        \textbf{\Framework-R} & \textbf{0.8156} & \textbf{0.7545} & \textbf{0.5913} & \textbf{0.4989} & \textbf{0.8361}  & \textbf{0.7924} &\textbf{0.6445} & \textbf{0.5397} & \textbf{0.8393} & \textbf{0.8033} & \textbf{0.6837} & \textbf{0.5887} \\           
        % (Gain) & 7.95\% & 10.22\% & 14.12\% & 18.36\% & 4.69\% & 5.73\% & 11.71\% & 18.14\% & 5.73\% & 6.18\% & 6.26\% & 11.70\% \\ 
        (Gain) & 17.04\% & 19.45\% & 22.82\% & 31.60\% & 10.63\% & 19.48\% & 19.06\% & 18.14\% & 19.06\% & 59.92\% & 77.72\% & 11.70\% \\ 
        \bottomrule[1pt]
    \end{tabularx}
    % \vspace*{-2em}
\end{table*}
%For the Beijing and Shanghai datasets, we randomly select 90\% of queries and their corresponding records as the training set and treat the remaining queries as the test set. From the training set, we randomly choose 10\% of queries as the validation set to tune the hyperparameters. For the Geo-Glue dataset~\cite{DBLP:conf/sigir/DingCXHLZX23}, we follow the provided splits for training, validation, and test data. 

% We evaluate the performance with six metrics: (1) averaged Normalized Discounted Cumulative Gain at top 1, (NDCG@1), (2) averaged Normalized Discounted Cumulative Gain at top 3 (NDCG@3), (3) averaged Normalized Discounted Cumulative Gain at top 5 (NDCG@5), (4) Recall at top 50 (Recall@50), (5) Recall at top 20 (Recall@20), and (6) Recall at top 10 (Recall@10).

\noindent\textbf{Effectiveness metric.} Following previous studies~\cite{DBLP:conf/sigir/DingCXHLZX23,liu2023effectiveness}, we use two %widely used 
metrics, i.e., the Recall and Normalized Discounted Cumulative Gain (NDCG), to evaluate the effectiveness.
%of the \tkskqs. 
Recall@$k$ evaluates the proportion of positive objects contained in the top-$k$ candidates for a given query. NDCG@$k$ considers the order of ground-truth objects in the retrieved objects, reflecting the quality of the ranking in the retrieved list. We assign the graded relevance of the result at position $i$ as $rel_{i} \in \{0,1\}$, where $rel_{i}=1$ when the object is relevant to the query, otherwise $rel_{i}=0$. More details can be found in \cite{liu2023effectiveness}. Specifically, the following metrics are utilized: Recall@10, Recall@20, NDCG@1, and NDCG@5. 
%to evaluate the effectiveness: 
%Recall at top-10 and top-20 (Recall@10, Recall@20), and NDCG at top-1 and top-5 (NDCG@1, NDCG@5).

% evaluate the effectiveness with four metrics: averaged Normalized Discounted Cumulative Gain at top 1 and 5 (NDCG@1, NDCG@5) and Recall at top 10 and 20 (Recall@10, Recall@20). NDCG is one of the most frequently used effectiveness metrics for ranking evaluation~\cite{liu2023effectiveness} and Recall is one of the most evaluation frequently used effectiveness metrics in information retrieval~\cite{katsogiannis2023survey}. NDCG@k\footnote{https://github.com/Lightning-AI/torchmetrics} is defined as $\text{NDCG}@k = \frac{\text{DCG}@k}{\text{IDCG}@k}$, where $\text{DCG}@k = \sum_{i=1}^{k} \frac{rel_i}{\log_2(i+2)}$, and $rel_i \in \{0,1\}$ is the graded relevance of the result at position i. $\text{IDCG}@k$ is the ideal discounted cumulative gain and acts as a normalization factor. $\text{Recall}@k$\footnote{https://github.com/castorini/anserini} is defined as $\text{Recall}@k = \frac{1}{|Q|} \sum_{q \in Q} \frac{\sum_{o^{+}\in D^{+}_{q}}1_{o^{+} \in R_{q}}} {{min(k,|D_{q}^{+}|)}}$. The $D_{q}^{+}$ is the ground truth set for query $q$ and the $R_{q}$ denotes top-K objects retrieved by a retrieval system for query $q$. There may be multiple positive objects $o^{+} \subset D^{+}_{q}$, $1_{o^{+} \in R_{q}}$ is an indicator that is 1 when $o^{+} \in R_{q}$ and 0 otherwise, and $Q$ denotes the test queries set. This metric is also referred as to all-positive-macro Recall@K.




\noindent\textbf{Relevance Model Baselines.} We compare our %proposed 
relevance model, denoted as \Framework-R, with existing state-of-the-art spatio-textual relevance models. %or state-of-the-art deep textual relevance models. We also modify the state-of-the-art textual relevance model DPR~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20} into DPR$_D$ to answer \tkskqs.
\begin{itemize}[leftmargin=*,topsep=0pt]
% \item BM25~\cite{DBLP:journals/ftir/RobertsonZ09}: A classic textual relevance model that is used in search engines. This method does not consider spatial relevance.
\item TkQ~\cite{congEfficientRetrievalTopk2009}: It uses traditional relevance model BM25~\cite{DBLP:journals/ftir/RobertsonZ09} to evaluate text relevance and treats $1-SDist(q.loc,o.loc)$ as spatial relevance. The weight parameter $\alpha$ is manually tuned from 0 to 1 with a footstep of 0.1, and the best effectiveness is achieved when $\alpha=0.4$ for all three datasets. %with footstep as 0.1 to yield the best effectiveness. We achieve the best effectiveness when $\alpha=0.4$ for all three datasets.  
\item PALM~\cite{DBLP:conf/aaai/ZhaoPWCYZMCYQ19}: This method employs deep neural networks for query-object spatio-textual relevance.
%to incorporate geographical location embeddings with semantic representations.
%, thereby estimating the relevance scores.  
\item DrW~\cite{liu2023effectiveness}: This is the 
%state-of-the-art 
newest deep relevance based method for answering \tkskqs. 
% \item DPR~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20}: This is a state-of-the-art textual relevance model for document retrieval. This method does not consider spatial relevance. 
% \item DPR$_{D}$: This method replaces the text relevance computation in DrW~\cite{liu2023effectiveness} with DPR~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20}. 
\item MGeo~\cite{DBLP:conf/sigir/DingCXHLZX23}: This is a recent deep learning based method for answering \tkskqs. Note that we cannot reproduce the experimental results reported in the paper by running the official code, and thus we use the evaluation results from the original paper.
\end{itemize}




% 

 
% \item 
% : This method employs a word-interaction module to evaluate the textual relevance, uses $1-SDist(q.loc,o.loc)$ as spatial relevance, and leverages a weight learning mechanism to determine weights. We select this method as a baseline since DrW is the state-of-the-art relevance model for answering \tkskqs. 
% \item KNRM$_D$: This method utilizes the text relevance model KNRM~\cite{DBLP:conf/sigir/XiongDCLP17} to serve as a relevance model to answer \tkskqs. It employs KNRM to evaluate text relevance, uses $1-SDist(q.loc,o.loc)$ to calculate spatial relevance, and tunes $\alpha$ to balance the two parts.

% \noindent\textbf{Baselines of \Index.} We compare our proposed index \Index with the following indexes:
% \begin{itemize}[leftmargin=*,topsep=0pt]
% \item TkQ: This method employs TkQ to retrieve top-$k$ objects for a given query and leverages IR-Tree~\cite{congEfficientRetrievalTopk2009} to accelerate this process. We set $k$ to 100 across three datasets. We do not further increase $k$ because, at $k=100$, the querying speed of IR-Tree is already an order of magnitude slower than our index. Different $k$ settings are demonstrated in Section~\ref{sec:exp-para}.
% \item IVF~\cite{jegouProductQuantizationNearest2011}: This method employs the k-means algorithm to cluster objects based on their text embeddings $o.emb$ and route a query to nearby clusters based on $q.emb$ to reduce the search space. The number of clusters $c$ and the number of clusters to route for a given query is the same as our index to make a fair comparison.
% \item LSH~\cite{johnson2019billion}: This method builds the Locality-Sensitive Hashing (LSH) index based on $o.emb$. It retrieves the top-$k$ relevant objects based on $q.emb$ by fetching similar embeddings in the same buckets. Following previous work~\cite{DBLP:conf/icml/NeyshaburS15}, we set the length of the hash code $nbits$ to 64. Different $nbits$ settings will be shown in Section~\ref{sec:exp-para}. We set top-$k$ to 20,000 across three datasets. We do not increase $k$ for the same reason above.
% \item HNSW~\cite{malkovEfficientRobustApproximate2020}: This method builds the Hierarchical Navigable Small World (HNSW) index based on $o.emb$. It retrieves the top-$k$ relevant objects by conducting beam searches over the proximity graph. Following previous work~\cite{malkovEfficientRobustApproximate2020}, we set the number of links $M$ to 48 and $efConstruction$ to 100. Different $M$ settings will be shown in Section~\ref{sec:exp-para}. We set top-$k$ to 20,000 across three datasets for the same reason above.
% \end{itemize}


% The HNSW index cannot be evaluated on the Geo-Glue dataset due to its large GPU memory requirements. 


% \noindent\textbf{Baselines of \Framework.} We compare \Framework with the following retrieve and rerank methods. 
\noindent\revision{\textbf{Index Baselines.} We compare our proposed index with existing state-of-the-art indexes. %to demonstrate its effectiveness and efficiency. 
Specifically, we select the IR-Tree~\cite{congEfficientRetrievalTopk2009} to accelerate the TkQ search, serving as an index baseline. As discussed in Section~\ref{sec:related}, existing ANNS indexes fall into two categories and our method belongs to the first category. We select the state-of-the-art ANNS indexes in the first category, i.e., IVF~\cite{jegouProductQuantizationNearest2011}, LSH~\cite{johnson2019billion}, and HNSW~\cite{malkovEfficientRobustApproximate2020}, as index baselines. For the second category of methods, such as product quantization based methods, their standalone efficiency is no better than a brute-force search\footnote{https://github.com/facebookresearch/faiss/issues/148}. Therefore, following previous work~\cite{jegouProductQuantizationNearest2011}, we choose IVFPQ as an index baseline, which integrates PQ with the IVF index from the first category and is considered as a state-of-the-art solution. As discussed  in Section~\ref{sec:motivations}, existing ANNS indexes are limited to considering only textual embeddings, neglecting the spatial factor. To mitigate this limitation, %we employ the DPR$_D$  model, which stands as the most effective baseline in our experiment, to rerank the objects retrieved by these ANNS indexes. Furthermore, 
we extend the IVF index to include both embedding and spatial factors%in the index construction phase
, which is denoted as IVF$_S$ index, as an index baseline. Similar to \Framework, which uses a retrieve and rerank pipeline, we utilize the aforementioned indexes to retrieve a subset of objects and then rerank the retrieved objects with our relevance model \Framework-R for a fair comparison. The integration of our proposed index and \Framework-R is \Framework, and the other methods are detailed below.}
\begin{itemize}[leftmargin=*,topsep=0pt]
\item \revision{TkQ+\Framework-R}: This method employs TkQ to retrieve top-$k$ objects and %then 
reranks these objects by \Framework-R.
\item \revision{IVF+\Framework-R}: This method constructs an IVF index over the embeddings produced by \Framework-R, and the objects within the selected index cluster are reranked by \Framework-R. Notably, this method requires two parameters: the number of clusters $c$, and the number of clusters to route for each query and object $cr$. It does not involve $k$. We set $c$ and $cr$ to be the same as our method across three datasets for a fair comparison.

\item \revision{IVF$_S$+\Framework-R}: This method follows the IVF+\Framework-R pipeline but diverges in the clustering approach. Instead of only applying k-means to text embeddings, this approach utilizes k-means on the weighted sum of both geo-location and text embedding factors. The weight $\alpha$ is manually tuned from 0 to 1 with a footstep of 0.1, and the best effectiveness is achieved when $\alpha=0.9$ for all these datasets.

\item  \revision{LSH+\Framework-R}: This method constructs an LSH index with the embeddings produced by \Framework-R, which retrieves the top-$k$ relevant objects by fetching similar embeddings in the same buckets, and reranks the retrieved objects by \Framework-R. Following previous work~\cite{johnson2019billion}, we set the length of the hash code $nbits$ to 128. 


\item  \revision{HNSW+\Framework-R}: This method constructs an HNSW index over the embeddings produced by \Framework-R, which retrieves the top-$k$ relevant objects by conducting beam searches over the proximity graph, and reranks the retrieved objects by \Framework-R. Following previous work~\cite{malkovEfficientRobustApproximate2020}, we set the number of links $M$ to 48 and $efConstruction$ to 100. 

\item  \revision{IVFPQ+\Framework-R}: This method integrates the IVF index with the product quantization technique~\cite{jegouProductQuantizationNearest2011} to retrieve objects. The retrieved objects are reranked by \Framework-R. We set the number of clusters $c$ to be the same as our index. Following the instruction~\cite{johnson2019billion}, we set the number of centroids $w$ to 32 and the number of bits $nbits$ to 8, the number of clusters to search $cr$ at 2. %Here, we do not set $cr$ the same as 
Here, we set a larger value for $cr$ than that in our index since the product quantization accelerates computations within clusters, allowing access to more clusters with comparable time costs. Notably, the maximal $k$ supported by the Faiss library is 2,048, therefore we set $k$ to 2,048 across three datasets. 
\end{itemize}
An important hyperparameter is $k$, which represents the number of objects retrieved by the indexes and reranks by LIST-R. To ensure a fair comparison, we set $k$ to 5,000 for the baselines that involve $k$ on the Beijing and Shanghai datasets, which is the average number of objects retrieved by our index per query. On the geo-glue dataset, $k$ is set to be 30,000 for the same reason above. \revision{To investigate the capability of \Framework to trade off effectiveness and efficiency, we evaluate the effect of the hyperparameter $cr$ and $k$ in Section~\ref{sec:exp-effectiveness-efficiency-tradeoff}.}%We evaluate the effect of $k$ in Section~\ref{sec:exp-efficiency}. \revision{To investigate the capability of \Framework to trade off effectiveness and efficiency, we vary the hyperparameter $cr$, which represents the number of clusters to route, from 1, 2, 3, to 4. For baselines that share the same hyperparameter with \Framework, i.e., IVF+\Framework-R, IVF$_S$+\Framework-R, and IVFPQ+\Framework-R, we maintain the same increment for $cr$. For other methods, we adjust the hyperparameter $k$, which represents the number of objects retrieved by the indexes, to be close to the number of objects retrieved by our proposed index, adjusting it from 5,000, 10,000, 20,000, to 40,000 on the Beijing and Shanghai datasets.
%For methods that do not involve the hyperparameter $k$, such as \Framework, IVF+\Framework-R, IVF$_S$+\Framework-R, and IVFPQ+\Framework-R, we adjust the hyperparameter $cr$, which denotes the number of clusters to route, from 1, 2, 3, 4, to 5 on Beijing and Shanghai datasets.
%The effectiveness-efficiency trade-off of \Framework and other baselines is largely influenced by the hyperparameter $k$, which represents the number of objects retrieved by the indexes and subsequently reranked by \Framework-R. To investigate \Framework and other methods's capability to trade off effectiveness and efficiency, 
% }


% An important hyperparameter is $k$, which represents the number of objects retrieved by the indexes and reranks by DPR$_D$. Specifically, on the Beijing and Shanghai datasets, for a fair comparison, we set $k$ to be 10,000, which is the average number of objects retrieved by our index per query. On the geo-glue dataset, $k$ is set to be 55,000 for the same reason above. We evaluate the effect of $k$ in Section~\ref{sec:exp-efficiency}.


% \begin{itemize}[leftmargin=*,topsep=0pt]
% \item TkQ+DPR$_D$: This method employs TkQ to retrieve top-$k$ objects and then reranks these objects by DPR$_D$. 


% \item  IVF+DPR$_D$: This method constructs an IVF index over the embeddings produced by DPR$_{D}$, %which employs the k-means algorithm to cluster object embeddings and route queries based on their distance to the centroids. 
% and the objects within the %routed 
% selected index cluster are reranked by DPR$_{D}$. Notably, this method requires two parameters: the number of clusters $c$, and the number of clusters to route for each query and object $cr$. It does not involve $k$. We set $c$ and $cr$ to be the same as our method across three datasets for a fair comparison. 
% % Different $c$ settings are evaluated in Section~\ref{sec:efficiency}.
% \item  IVF$_S$+DPR$_D$: This method follows the IVF+DPR$_D$ pipeline but diverges in the clustering approach. Instead of only applying k-means to text embeddings, this approach utilizes k-means on the weighted sum of both geo-location and text embedding factors. The weight $\alpha$ is manually tuned from 0 to 1 with a footstep of 0.1, and the best effectiveness is achieved when $\alpha=0.9$ for all these datasets.

% \item  LSH+DPR$_D$: This method constructs an LSH index with the embeddings produced by DPR$_{D}$, which retrieves the top-$k$ relevant objects by fetching similar embeddings in the same buckets, and reranks the retrieved objects by DPR$_{D}$. Following previous work~\cite{johnson2019billion}, we set the length of the hash code $nbits$ to 128. 


% \item  HNSW+DPR$_D$: This method constructs an HNSW index over the embeddings produced by DPR$_{D}$, which retrieves the top-$k$ relevant objects by conducting beam searches over the proximity graph, and reranks the retrieved objects by DPR$_{D}$. Following previous work~\cite{malkovEfficientRobustApproximate2020}, we set the number of links $M$ to 48 and $efConstruction$ to 100. 

% \item  IVFPQ+DPR$_D$: This method integrates the IVF index with the product quantization technique~\cite{jegouProductQuantizationNearest2011} to retrieve objects. The retrieved objects are reranked by DPR$_{D}$. We set the number of clusters $c$ to be the same as our index. Following the instruction~\cite{johnson2019billion}, we set the number of centroids $w$ to 32 and the number of bits $nbits$ to 8, the number of clusters to search $cr$ at 4. %Here, we do not set $cr$ the same as 
% Here, we set a larger value for $cr$ than that in our index since the product quantization accelerates computations within clusters, allowing access to more clusters with comparable time costs. Notably, the maximal $k$ supported by the Faiss library is 2,048, therefore we set $k$ to 2,048 across three datasets. 
% \end{itemize}



% Due to the page limitation, we demonstrate the effect of key parameters for all these indexes in our full version paper\footnote{https://github.com/Heisenberg-Yin/LIST}.

% {\color{blue} We exclude quantization-based methods like IVFPQ~\cite{jegouProductQuantizationNearest2011} from our baseline index consideration. IVFPQ utilizes the IVF index to reduce the search space and employs product quantization techniques to expedite the search process, while our proposed index focuses on effectively reducing the search space, as discussed in Section~\ref{sec:related}. Including IVFPQ or other quantization-based methods in the baseline would lead to an unfair comparison.}





% Additionally, Faiss heavily uses OpenMP for multi-threading while our method's implementation does not have such optimization. We set the number of threads of Faiss to 1 for fair comparisons.

% \begin{table*}[t]
% % \vspace*{-1em}
%     \centering
%     \caption{Comparison of retrievers across three datasets.}
%     % \vspace*{-0.5em}
%     \label{tab:effective}
%     % \small
%     \renewcommand{\arraystretch}{1.5} % 控制行高
%     \setlength{\arrayrulewidth}{0.5pt}
%     \begin{tabularx}{1\textwidth}{>{\centering}m{2.5cm}*{4}{X}*{4}{X}*{4}{X}}
%         \toprule[1pt]
%         \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Beijing}} & \multicolumn{4}{c} {\textbf{Shanghai}} & \multicolumn{4}{c} {\textbf{Geo-Glue}} \\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
%         & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}}  &
%         \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
%         \cmidrule(lr){10-11} \cmidrule(lr){12-13}
%         & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1} \\
%         \midrule[1pt]
%         % TkQ  & 0.5740 & 0.5283 & 0.4111 & 0.3302 & {0.6746} & 0.6380 & 0.5044 & 0.4009 & 0.5423 & 0.5023 & 0.3847 & 0.3051 \\         
%         % TkQ+DrW  & {0.6211} & {0.5852} &  {0.4646} & {0.3848} & {0.7014} & {0.6666} & {0.5195} & {0.4120} & 0.5023 & 0.4447 & 0.3101  & 0.2268 \\      
%         TkQ+DPR$_D$ & \underline{0.7263} & \underline{0.6633} & \underline{0.5056} & \underline{0.4145} & \underline{0.7717} & \underline{0.7348} & \underline{0.5742} & \underline{0.4556} & \underline{0.7357} & \underline{0.7012} & \underline{0.5797} & \underline{0.4878} \\  
        
%         IVF+DPR$_{D}$ & 0.5461 & 0.4954 & 0.3771 & 0.3103  & 0.4965 & 0.4717 & 0.3713 & 0.3000 & {0.4720} & {0.4535} & {0.3835} & {0.3274} \\
%         IVF$_{S}$+DPR$_{D}$ & 0.4126 & 0.3714 & 0.3025 & 0.2415  & 0.4174 & 0.3812 & 0.2960 & 0.2101 & {0.3921} & {0.3714} & {0.3011} & {0.2419} \\        
%         % LSH+DPR$_{D}$ & 0.6283 & 0.5747 & 0.4441 & 0.3703 & 0.6651 & 0.6281 & 0.4935 & 0.3992 & {0.4304} & {0.4163} & {0.3625}  & {0.3187}\\ 64
%         LSH+DPR$_{D}$ & {0.5473} & {0.5057} & {0.3973} & {0.3385} & {0.5356} & 0.5097 & 0.4135 & 0.3453 & {0.6686} & {0.6433} & {0.5445} & {0.4661} \\ 
%         HNSW+DPR$_{D}$ & 0.6267 & 0.5828 & 0.4545 & 0.3765 & 0.5527 & 0.5270 & 0.4182 & 0.3432 & 0.5009 & 0.4807 & 0.4066 & 0.3468 \\
%         IVFPQ+DPR$_{D}$ & 0.7064 & 0.6400 & 0.4872 & 0.4002 & 0.7184 &0.6765 & 0.5257 & 0.4188& {0.6997} & {0.6724} & {0.5650} & {0.4791}\\        
%         % \midrule
%         % TkQ+\Model & \underline{0.6514} & \underline{0.6315} & \underline{0.5312} & \underline{0.4639} & \underline{0.7316} & \underline{0.7069} & \underline{0.5957} & \underline{0.5117}  & \underline{0.6180}  & \underline{0.6132}  & \underline{0.5552} & \underline{0.4993}  \\  
        
%         % % TkQ+\Model (500) & \underline{0.7066} & \underline{0.6742} & \underline{0.5510} & \underline{0.4749} & \underline{0.7672} & \underline{0.7353} & \underline{0.6156} & \underline{0.5262}  &   &   &   &   \\  
        
%         % IVF+\Model & 0.6405 & 0.5944 & 0.4671 & 0.3960 & 0.6032 & 0.5758 & 0.4746 & 0.4010 & 0.5394 & 0.5204 & 0.4512 & 0.3969 \\ 
%         % LSH+\Model & 0.6234 & 0.5842 &  0.4744 &  0.4139 & 0.5121 & 0.4912 & 0.4171 & 0.3678 & 0.5444 & 0.5301 & 0.4715 & 0.4212 \\ 
%         % HNSW+\Model & 0.6005 & 0.5698 & 0.4665 & 0.4070 & 0.6087 & 0.5809 & 0.4901 & 0.4263 & N/A & N/A & N/A  & N/A \\
        
%         % TkQ+KNRM$_D$ & 0.5190 & 0.4728 & 0.3547 & 0.2894 & 0.6199 & 0.5817 & 0.4630 & 0.3800 & 0.4619 & 0.4004 & 0.2678 & 0.1938 \\  
   
%         % TkQ+DrW (500) & {0.6568} & {0.6115} &  {0.4738} & {0.3867} & {0.7321} & {0.6931} & {0.5359} & {0.4217} & 0.5023 & 0.4447 & 0.3101  & 0.2268 \\ 
        

        
%         % MGeo & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A &  &  &  &  \\       
%         \midrule
%         \textbf{\Framework} & \textbf{0.7711} & \textbf{0.7170} & \textbf{0.5668} & \textbf{0.4812} & \textbf{0.7721}  & \textbf{0.7401} &\textbf{0.6099} & \textbf{0.5139} & \textbf{0.8250} & \textbf{0.7909} & \textbf{0.6747} & \textbf{0.5815} \\    
%         % \textbf{\Framework} & \textbf{0.7711} & \textbf{0.7170} & \textbf{0.5668} & \textbf{0.4812} & \textbf{0.7951}  & \textbf{0.7415} &\textbf{0.6074} & \textbf{0.5119} & \textbf{0.8250} & \textbf{0.7909} & \textbf{0.6747} & \textbf{0.5815} \\         
%         % \midrule
%         (Gain) & 5.63\% & 7.95\% & 10.70\% & 15.32\% & 0.05\% & 0.72\% & 6.21\% & 12.54\% & 12.13\% & 12.79\% & 16.38\% & 19.21\% \\  
%         \bottomrule[1pt]
%     \end{tabularx}
%     % \vspace*{-2em}
% \end{table*}

\noindent\textbf{Implementations.} The relevance model and the index are trained using Pytorch. During the query phase, the index and all relevance models are inferred in C++ by the ONNX system\footnote{https://github.com/onnx/onnx}. In our proposed relevance model, we utilize the bert-base-Chinese pre-trained model\footnote{https://huggingface.co/bert-base-chinese} from the huggingface Library~\cite{wolf2019huggingface} as encoders, which is the same as previous work~\cite{liu2023effectiveness,DBLP:conf/sigir/DingCXHLZX23}. \revision{The hyperparameter settings of \Framework are detailed in Table~\ref{tab:hyper}.} Specifically, the spatial footstep controller $t$ of $\mathcal{T}$ is set to 1000 for all three datasets. The hyperparameters to control the generation of pseudo labels, $\text{neg}_\text{start}$ and $\text{neg}_\text{end}$, are set to 50,000 and 55,000 for the Beijing dataset, 60,000 and 65,000 for the Shanghai dataset, and 180,000 and 181,000 for the Geo-Glue dataset.
 %The $\lambda$ is set to be 0.6.
%for the Beijing dataset 0.7 for the Shanghai dataset, and 0 for the geo-glue dataset.
%\footnote{Due to numerous objects and relatively fewer queries in the geo-glue dataset, many of its clusters lack associated routed queries, and reassigning the objects within these clusters harms the efficiency significantly.}. 
We empirically set the cluster number $c$ to approximately $\frac{n}{10,000}$, i.e.,  20 for the Beijing and Shanghai datasets and 300 for the Geo-Glue dataset. This is because ranking 10,000 objects by the relevance model is computationally feasible and does not notably compromise effectiveness. The number of clusters to route $cr$ for queries and objects is set to 1 by default, with different $cr$ settings shown in Section~\ref{sec:exp-effectiveness-efficiency-tradeoff}. The implementations of DrW are from publicly available source codes, and we make use of the implementation of IVF, LSH, IVFPQ, and HNSW provided by the Faiss library~\cite{johnson2019billion}, while others are implemented by ourselves. The Faiss library is implemented in C++, providing a fair comparison with our index. %Additionally, Faiss heavily uses OpenMP for multi-threading while our method's implementation does not have such optimization. We set the number of threads of Faiss to 1 for fair comparisons. 
Our default experiment environment is CPU: Intel(R) Core(TM) i9-10900X CPU@3.70GHz, Memory: 128G, and GPU: V100 32GB. 




\begin{figure*}[!t]
\centering
\subcaptionbox{Beijing\label{fig:exp-beijing}}{
\includegraphics[width=0.9\textwidth]{fig/beijing_tradeoff.pdf}
}
\subcaptionbox{Shanghai\label{fig:exp-shanghai}}{
\includegraphics[width=0.9\textwidth]{fig/shanghai_tradeoff.pdf}
}
\subcaptionbox{Geo-Glue\label{fig:exp-geoglue}}{
\includegraphics[width=0.9\textwidth]{fig/geoglue_tradeoff.pdf}
}
\caption{\revision{The effectiveness-efficiency trade-off results (upper and right is better).}}
\label{fig:exp-effective-efficiency}
\end{figure*}

\subsection{Effectiveness of Proposed Relevance Model (RQ1)}
\label{sec:exp-effectiveness}
\noindent\textbf{Effectiveness of Relevance Model \Framework-R.} To validate our proposed relevance model's effectiveness, denoted as \Framework-R, we compare it with other relevance models across the three datasets. All relevance models perform a brute-force search over the entire dataset to identify the top-k objects. Table~\ref{tab:relevance_model} reports the effectiveness of the evaluated methods. DrW and PLAM cannot be evaluated on the Geo-Glue dataset via brute-force search because of their slow querying speed, requiring more than a day for evaluation. We have the following findings: (1) \Framework-R consistently outperforms all the baseline models on all three datasets across every metric. Specifically, \Framework-R achieves up to a 31.60\% improvement over the best baseline on NDCG@1 and up to a 59.92\% improvement on recall@10. (2) Traditional ranking methods are less effective than deep relevance models. On the three datasets, TkQ is outperformed by DrW. %and DPR$_D$. 
This can be attributed to the word mismatch issue discussed in Section~\ref{sec:motivations}. Notably, PALM is outperformed by TkQ, which is consistent with the results reported by~\cite{liu2023effectiveness}. %(3) Directly applying the dual-encoder model to our task is less effective. On the Beijing and Shanghai datasets, DPR is outperformed by TkQ, which is caused by the ignorance of spatial relevance. DPR's enhanced effectiveness on the geo-glue dataset can be attributed to the property of the dataset, where most queries are address descriptions~\cite{DBLP:conf/sigir/DingCXHLZX23}. 

\begin{figure*}[!t]
\centering
\subcaptionbox{Beijing\label{fig:exp-beijing-k}}{
\includegraphics[width=0.9\textwidth]{fig/beijing_tradeoff_k.pdf}
}
\subcaptionbox{Shanghai\label{fig:exp-shanghai-k}}{
\includegraphics[width=0.9\textwidth]{fig/shanghai_tradeoff_k.pdf}
}
\caption{\revision{The Effectiveness-Speed trade-off curve varies with the number of objects retrieved (top-$k$) and the number of clusters to route ($cr$) (up and right is better).}}
\label{fig:exp-effective-efficiency-tradeoff}
\end{figure*}

\subsection{\revision{Effectiveness-Efficiency Trade-off of Proposed Index (RQ2)}}
\label{sec:exp-effectiveness-efficiency-tradeoff}

\noindent\revision{\textbf{Effectiveness-efficiency trade-off of \Framework.} We investigate the effectiveness-efficiency trade-off of \Framework by comparing it with the state-of-the-art index baselines, which all use our relevance model. The evaluation results are shown in Figure~\ref{fig:exp-effective-efficiency}, where LIST-R represents the brute-force search using our relevance model. We have the following findings: (1) Overall, \Framework consistently outperforms all baselines, offering the best trade-off between effectiveness and efficiency across all three datasets. Specifically, compared to 
%the most effective baseline, TkQ+LIST-R, 
LIST-R, \Framework is an order of magnitude faster on the Beijing and Shanghai datasets and three orders of magnitude faster on the Geo-Glue dataset. While most ANNS indexes have similar runtime to \Framework, their effectiveness falls short. %IVF+LIST-R and IVFPQ+LIST-R have similar runtimes as \Framework. However, their effectiveness is worse than \Framework. 
(2) Directly applying ANNS indexes to spatial keyword queries results in a significant drop in effectiveness. Compared to LIST-R, which uses brute-force search, existing ANNS indexes sacrifice considerable effectiveness for improved efficiency. This could be attributed to the fact that these ANNS indexes do not consider the spatial factor. %Compared with other ANNS indexes-based methods, TkQ+LIST-R offers better effectiveness across the three datasets. 
(3) When TkQ is used as an index baseline, it %exhibits a 
is significantly slower. The reason is that the IR-Tree is not designed to retrieve a large number of objects.  
%exploits a priority queue, using the bottom object to prune lower-scoring objects. 
As the 
%queue size (
hyperparameter $k$ increases, the IR-Tree's pruning ability declines, which is consistent with previous empirical results~\cite{congEfficientRetrievalTopk2009}. (4) Simply modifying the existing ANNS index to incorporate the spatial factor is even less effective. IVF+LIST-R consistently outperforms IVF$_S$+LIST-R on the three datasets. This confirms that manually assigning a weight to balance the two factors is 
%both laborious and 
ineffective. }



\noindent\textbf{Trade-off Study by varying the number of objects retrieved (top-$k$) and the number of clusters to route ($cr$).} \revision{We examine \Framework's ability to trade off effectiveness and efficiency. %under the different number of clusters to route $cr$ settings. 
Here, we vary the hyperparameter $cr$, which represents the number of clusters to route, from 1, 2, to 3 on the Beijing and Shanghai datasets. For baselines that share the same hyperparameter with \Framework, i.e., IVF+\Framework-R, IVF$_S$+\Framework-R, and IVFPQ+\Framework-R, we maintain the same increment for $cr$. For other methods, we adjust the hyperparameter $k$, which represents the number of objects retrieved by the indexes, to be close to the number of objects retrieved by our proposed index, adjusting it from 5,000, 10,000, to 20,000 on the Beijing and Shanghai datasets. For TkQ+\Framework-R, due to its slow query processing speed, we adjust $k$ from 100, 500, 1,000, 5,000, and 10,000 to 20,000. We present the trade-off results in Figure~\ref{fig:exp-effective-efficiency-tradeoff}. We have the following findings: (1) \Framework consistently outperforms other methods, providing a better trade-off between effectiveness and efficiency. (2) Compared to other methods, the effectiveness of TkQ+LIST-R increases more slowly as $k$ increases, while the time overhead rises significantly. This is due to the word mismatch issue discussed in Section~\ref{sec:motivations}. Many relevant objects without word overlap with the query remain hard to retrieve as $k$ increases. (3) HNSW+LIST-R 
%exhibits almost constant results. 
is almost not affected by the number of retrieved objects. 
This is because HNSW builds a sparse proximity graph, limiting the reachable objects for each query. Therefore, when $k$ exceeds the number of reachable objects, its performance remains unchanged.}

 


% \noindent\textbf{Effectiveness of \Framework.} We investigate the effectiveness of \Framework by comparing it with the state-of-the-art baselines. The evaluation results are reported in Table~\ref{tab:effective}. We have the following findings:
% (1) Directly applying ANNS indexes in TkQ task results in severe effectiveness degradation. These inferior results can be attributed to the ignorance of the spatial factor by these ANNS indexes. Compared with other ANNS indexes-based methods, TkQ+DPR$_D$ offers better effectiveness across the three datasets. 
% (2) Overall, \Framework significantly outperforms all the baselines, achieving the highest scores on all datasets. Compared with the strongest baseline TkQ+DPR$_D$, \Framework achieves up to 12.13\% improvements on Recall@10 metric and 19.20\% on NDCG@1 metric. (3) Simply modifying the existing ANNS index to incorporate the spatial factor is even less effective. IVF+DPR$_D$ outperforms IVF$_S$+DPR$_D$ by a large margin. This confirms that manually assigning a weight to balance the two factors is both laborious and ineffective.


% \begin{table}[h]
%     % \vspace*{-2em}
%     \centering
%     \caption{Query runtime on three datasets (ms).}
%  %   \vspace*{-0.5em}
%     \label{tab:runtime}
%     \renewcommand{\arraystretch}{1.2} % 控制行高
%     \setlength{\arrayrulewidth}{0.5pt}
%     % \small
%     \begin{tabularx}{0.5\textwidth}{>{\centering}m{2.5cm}*{3}{X}}
%     \toprule[1pt]
%     \multirow{2}{*}{} & Beijing & Shanghai & Geo-Glue\\
%     \midrule[1pt]
%     TkQ & 6.3 & 6.5 & 1,178.0\\
%     TkQ+DPR$_D$ & 86.3 & 84.9 & 5,412.3\\
%     IVF+DPR$_D$ & \underline{2.9} & \underline{2.9} & \underline{4.0} \\ 
%     LSH+DPR$_D$ & 5.2 & 5.1 & 31.1 \\ 
%     HNSW+DPR$_D$ & 7.3 & 6.5 & 14.6 \\
%     IVFPQ+DPR$_D$ & 3.6 & 3.7 & 5.2 \\
%     \midrule
%     \textbf{LIST} & \textbf{3.0} & \textbf{3.0} & \textbf{5.1} \\  
%     \bottomrule[1.5pt]
%   \end{tabularx}
%   % \vspace*{-1em}
% \end{table}
% \vspace*{-1em}
% \subsection{Efficiency Study (RQ2)}
% \label{sec:exp-efficiency}
% \noindent\textbf{Runtime of \Framework.} We investigate the querying speed of \Framework by comparing it with the state-of-the-art baselines. During the query phase, our proposed index, IVF, LSH, IVFPQ, and HNSW remain in the GPU, while IR-Tree remains in the memory. The total runtime is computed by calculating the average time cost of 5,000 randomly sampled queries from the test query set. We present the total runtime of different methods in Table~\ref{tab:runtime}. Based on the experimental results, we have the following findings: (1) Compared with the most effective baselines, i.e., TkQ+DPR$_D$, \Framework is one order of magnitude faster on the Beijing and Shanghai datasets and three orders of magnitude faster on the Geo-Glue dataset. (2) IVF+DPR$_{D}$ and IVFPQ+DPR$_{D}$ have similar runtimes as \Framework. However, their effectiveness is much worse than \Framework as stated in Table~\ref{tab:effective}. Specifically, compared with the IVFPQ+DPR$_{D}$, \Framework achieves an improvement of up to 22.70\% on the NDCG@1 metric across the three datasets. Compared with the IVF+DPR$_{D}$ baseline, we observe an improvement of up to 77.61\% on the NDCG@1 metric across the three datasets. (3) The TkQ+DPR$_D$ exhibits a significantly slower querying speed than TkQ across three datasets. The reason is that IR-Tree exploits a priority queue, using the bottom object to prune lower-scoring objects. As the queue size (hyperparameter $k$) increases, the IR-Tree's pruning ability declines, aligning with previous empirical results~\cite{congEfficientRetrievalTopk2009}. (4) On the Beijing and Shanghai datasets, the querying speed of TkQ aligns with previous experiments~\cite{DBLP:journals/pvldb/ChenCJW13} on similar-sized datasets. However, on the Geo-Glue dataset, TkQ exhibits a slower querying speed compared to that reported in previous experiments on similar-sized datasets. This is due to the coordinate adjustments mentioned in Section~\ref{sec:exp-setup}, which results in many objects having identical locations. This affects the IR-Tree's pruning capability, which relies heavily on the exact distance between queries and objects to prune low-score objects. In conclusion, the proposed \Framework not only delivers exceptional effectiveness but also achieves remarkable efficiency.
% \begin{figure}[t]
% % \vspace*{-1.5em}
% \begin{center}
% \subfigure[\centering {Beijing Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_beijing.pdf}
% }
% }
% % \vspace*{-1em}
% \subfigure[\centering {Beijing Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_beijing.pdf}
% }
% }
% % \vspace*{-1em}
% \subfigure[\centering {Shanghai Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_shanghai.pdf}}
% }
% \subfigure[\centering {Shanghai Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_shanghai.pdf}}
% }
% % \vspace*{-0.5em}
% %\caption{The Effectiveness-Speed trade-off curve when varying the number of objects to retrieve top-$k$ and the number of cluster $c$ (up and right is better).}
% \caption{The Effectiveness-Speed trade-off curve varies with the number of objects retrieved (top-$k$) and the number of clusters ($c$) (up and right is better).}
% % \vspace*{-1.5em}
% \label{fig:trade-off-1}
% \end{center}
% \end{figure}


%\noindent\textbf{Trade-off Study by varying $k$, $c$ and $nprobe$.} We examine \Framework's ability to trade off effectiveness and efficiency under different hyperparameter settings. Specifically, on the Beijing and Shanghai datasets, we set the hyperparameter cluster number $c$ of \Framework and IVF+DPR$_D$ from 5, 10, 20, 50, to 100. For other baselines, i.e. LSH+DPR$_D$, HNSW+DPR$_D$, TkQ+DPR$_D$, we set hyperparameter top-$k$ from 1,000, 5,000, 10,000, 20,000 to 40,000. For the IVFPQ baseline, as the maximal value of top-$k$ is limited, we tune the number of clusters to search $nprobe$ from 2,4,6,8 to 10. Other hyperparameter settings are fixed. We present the trade-off study results on the NDCG@1 and Recall@10 metrics for the Beijing and Shanghai datasets in Figure~\ref{fig:trade-off-1} while other metrics and datasets have similar results. We have the following findings: (1) \Framework outperforms other methods on both effectiveness and efficiency. This demonstrates \Framework's capability of maintaining effectiveness while accelerating querying speed. (2) On the Shanghai dataset, TkQ+DPR$_D$ exhibits effectiveness comparable to that of \Framework, while being one order of magnitude slower than our approach. (3) The effectiveness of TkQ+DPR$_D$ is consistent as $k$ increases while time overhead increases significantly. This is due to the word mismatch issue discussed in Section~\ref{sec:motivations}. Many relevant objects without word overlap with the query remain hard to retrieve as $k$ increases. (4) HNSW+DPR$_D$ exhibits almost constant results. This is because HNSW builds a sparse proximity graph, limiting the reachable objects for each query. Therefore, when $k$ exceeds the number of reachable objects, its performance remains unchanged.

%\begin{figure}[!htbp]\vspace*{-1em}
%\begin{center}
% \subfigure[\centering \textbf{Beijing Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_beijing.pdf}
% }
% }
% \vspace*{-1em}
% \subfigure[\centering \textbf{Beijing Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_beijing.pdf}
% }
% }
% \vspace*{-1em}
% \subfigure[\centering \textbf{Shanghai Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_shanghai.pdf}}
% }
% \subfigure[\centering \textbf{Shanghai Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_shanghai.pdf}}
% }
% % \vspace*{-0.5em}
% \caption{The Effectiveness-Speed trade-off curve when varying $k$, $c$ and $nprobe$ (up and right is better).}
% \vspace*{-2em}
% \label{fig:trade-off-1}
% \end{center}
% \end{figure}





% \noindent\textbf{Trade-off Study by varying the number of objects retrieved (top-$k$) and the number of clusters ($c$).} We examine \Framework's ability to trade off effectiveness and efficiency under the different number of cluster $k$ settings. Specifically, on the Beijing and Shanghai datasets, we set the hyperparameter cluster number $c$ of \Framework, IVF+DPR$_D$, and IVFPQ+DPR$_D$ from 5, 10, 20, 50, to 100. For other baselines, i.e., LSH+DPR$_D$, HNSW+DPR$_D$, and TkQ+DPR$_D$, we set hyperparameter the number of objects retrieved (top-$k$) from 40,000, 20,000, 1,0000, 5,000 to 2,000. This ensures the number of objects retrieved for reranking is consistent across different baselines, leading to a fair comparison. Other hyperparameter settings are fixed. We present the trade-off results on the NDCG@1 and Recall@10 metrics for the Beijing and Shanghai datasets in Figure~\ref{fig:trade-off-1} while other metrics and datasets have similar results. We have the following findings: (1) \Framework outperforms other methods on both effectiveness and efficiency. This demonstrates \Framework's capability of maintaining effectiveness while accelerating querying speed. %(2) On the Shanghai dataset, TkQ+DPR$_D$ exhibits effectiveness comparable to that of \Framework, while being one order of magnitude slower than our approach. 
% (2) The effectiveness of TkQ+DPR$_D$ is consistent as $k$ increases while time overhead increases significantly. This is due to the word mismatch issue discussed in Section~\ref{sec:motivations}. Many relevant objects without word overlap with the query remain hard to retrieve as $k$ increases. (3) HNSW+DPR$_D$ exhibits almost constant results. This is because HNSW builds a sparse proximity graph, limiting the reachable objects for each query. Therefore, when $k$ exceeds the number of reachable objects, its performance remains unchanged.
% }

% The effectiveness of TkQ+DPR$_D$ remains unchanged when $k$ increases while the time overhead significantly increases. This is because many relevant objects cannot be retrieved by TkQ due to word mismatch issues discussed in Section~\ref{sec:motivations}. As a result, increasing $k$ does not lead to better effectiveness. /
% The runtime of \Framework eventually converges to the inference time of the query encoder and the index, which is a constant millisecond value across different datasets.

% On both datasets, \Framework is not only more effective but also more efficient compared with all other baselines.

% we set hyperparameters $k$ from 128, 256, 512, 1,024, and 2,048 across three datasets.


% We set  For other DPR$_D$ based baselines, we set the same hyperparameter across the three datasets. Specifically, we set hyperparameter $nbits$ of LSH+DPR$_D$ from 32, 64, 96, 128, to 256, hyperparameter $M$ of HNSW+DPR$_D$ from 32, 48, 64, 128, to 256, and hyperparameter $k$ of IR-Tree+DPR$_D$ from 50, 100, 200, 300, to 500. 


% According to the experiment results, 

% 




% \begin{figure}[!htbp]\vspace*{-2em}
% \begin{center}
% \subfigure[\centering \textbf{Beijing Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_beijing-2.pdf}
% }
% }
% \vspace*{-1em}
% \subfigure[\centering \textbf{Beijing Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_beijing-2.pdf}
% }
% }
% \vspace*{-1em}
% \subfigure[\centering \textbf{Shanghai Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_ndcg_shanghai-2.pdf}}
% }
% \subfigure[\centering \textbf{Shanghai Dataset}]{
% \raisebox{-1.5em}{\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_recall_shanghai-2.pdf}}
% }
% % \vspace*{-0.5em}
% \caption{The Effectiveness-Speed trade-off curve when varying $nbits$, $M$, $nc$ and $c$ (up and right is better).}
% \vspace*{-2em}
% \label{fig:trade-off-2}
% \end{center}
% \end{figure}


% \begin{figure}[h]
% % \vspace*{-1.5em}
% \begin{center}
% \subfigure[\centering {Beijing Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_nc_k_ndcg_beijing.pdf}}
% }
% % \vspace*{-1em}
% \subfigure[\centering {Beijing Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_nc_k_recall_beijing.pdf}}
% }
% % \vspace*{-1em}
% \subfigure[\centering {Shanghai Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/tradeoff_plot_nc_k_ndcg_shanghai.pdf}}
% }
% \subfigure[\centering {Shanghai Dataset}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]
% {fig/tradeoff_plot_nc_k_recall_shanghai.pdf}}
% }
% % \vspace*{-0.5em}
% % \caption{The Effectiveness-Speed trade-off curve when varying $k$ and $cr$ (up and right is better).}
% \caption{The Effectiveness-Speed trade-off curve varies with the number of objects retrieved (top-$k$) and the number of clusters to route ($cr$) (up and right is better).}
% % \vspace*{-1.5em}
% \label{fig:trade-off-2}
% \end{center}
% \end{figure}
% {\color{red}
% \noindent\textbf{Trade-off Study by varying the number of objects retrieved (top-$k$) and the number of clusters to route ($cr$).} We further investigate the impact of the number of clusters $cr$ to route queries and objects. We vary $cr$ from 1, 2, 3, to 4 for IVF+DPR$_D$ and our index, from 4, 5, 6, to 7 for IVFPQ+DPR$_D$. For other baselines, we set hyperparameter the number of objects retrieved (top-$k$) from 10,000, 20,000, 3,0000, to 4,0000 for a fair comparison like the previous trade-off study. Other hyperparameter settings are fixed. Similarly, we report the trade-off results on NDCG@1 and Recall@10 metrics for the Beijing and Shanghai datasets in Figure~\ref{fig:trade-off-2}. According to the experiment results, \Framework outperforms other methods in both effectiveness and efficiency under different $cr$ settings. Increasing $cr$ can enhance effectiveness, but it also leads to higher latency. In practice, users can adjust this parameter according to their needs.


%whether \Framework can still outperform other methods under different index settings. For LSH+DPR$_D$, we vary the hyperparameter $nbits$, representing the length of the hash code in the LSH index, from 32, 64, 128, 256 to 384. For HNSW+DPR$_D$, we vary the hyperparameter $M$, denoting the number of links $M$ for the HNSW index, from 12, 24, 48, 56 to 64. For IVFPQ+DPR$_D$, we vary the hyperparameter $nc$, representing the number of centroids in the IVFPQ index, from 8, 16, 32, 48 to 64. For \Framework and IVF+DPR$_D$, we vary hyperparameter $c$, which is the number of clusters, the same setting as the previous study. The other settings are fixed. Similarly, for the Beijing and Shanghai datasets, we report the trade-off study on NDCG@1 and Recall@10 metrics in Figure~\ref{fig:trade-off-2}. According to the experiment results, \Framework outperforms other methods in both effectiveness and efficiency under different index settings.
% }
% \noindent\textbf{Trade-off Study by varying $nbits$, $M$, $nc$ and $c$.} In this study, we investigate whether \Framework can still outperform other methods under different index settings. For LSH+DPR$_D$, we vary the hyperparameter $nbits$, representing the length of the hash code in the LSH index, from 32, 64, 128, 256 to 384. For HNSW+DPR$_D$, we vary the hyperparameter $M$, denoting the number of links $M$ for the HNSW index, from 12, 24, 48, 56 to 64. For IVFPQ+DPR$_D$, we vary the hyperparameter $nc$, representing the number of centroids in the IVFPQ index, from 8, 16, 32, 48 to 64. For \Framework and IVF+DPR$_D$, we vary hyperparameter $c$, which is the number of clusters, the same setting as the previous study. The other settings are fixed. Similarly, for the Beijing and Shanghai datasets, we report the trade-off study on NDCG@1 and Recall@10 metrics in Figure~\ref{fig:trade-off-2}. According to the experiment results, \Framework outperforms other methods in both effectiveness and efficiency under different index settings.



\noindent\textbf{Memory Consumption of \Framework.} 
The memory consumption of LIST is composed of three parts: the memory used by the proposed relevance model, the memory used by the proposed index, and the memory used for object text embeddings that are produced in advance. The experiment results are presented in Table~\ref{tab:memory}, which demonstrates the remarkable memory efficiency of \Framework. Compared with LSH+LIST-R, TkQ+LIST-R, and HNSW+LIST-R, \Framework requires less memory. The reason is that our index stores only a lightweight MLP $c$-cluster classifier. This storage requirement is less than the memory consumption of the proximity graph of HNSW, hash tables of LSH, and the inverted file of the IR-Tree.
\begin{table}[h]
    % \vspace*{-0.5em}
    \centering
     \caption{Memory usage on three datasets (MB).}
    % \vspace*{-0.5em}
    \label{tab:memory}
    \renewcommand{\arraystretch}{1.5} % 控制行高
    \setlength{\arrayrulewidth}{0.5pt}
    \small
    \begin{tabularx}{0.5\textwidth}{>{\centering}m{2.5cm}*{3}{X}}
    \toprule[1pt]
    \multirow{2}{*}{} & Beijing & Shanghai & Geo-Glue\\
    \midrule[1pt]
    % KNRM$_D$  & 188 & 154 & 589 \\ 
    % DrW & 189 & 155 & 592\\
    % DPR$_D$ & 508 & 505 & 8,494 \\
    % TkQ & 211 & 197 & 2,951 \\
    % TkQ+DrW & 400 & 352 & 3,543 \\
    TkQ+LIST-R & 719 & 857 & 12,037\\
    IVF+LIST-R & 508 & 505 & 8,510 \\  
    LSH+LIST-R & 513 & 511 & 8,638 \\ 
    HNSW+LIST-R & 548 & 545 & 9,427 \\ 
    IVFPQ+LIST-R & 508 & 505 & 8,520 \\  
    \midrule
    \textbf{\Framework} & 508 & 505 & 8,515 \\    
    \bottomrule[1pt]
  \end{tabularx}
  % \vspace*{-1.5em}
\end{table}

% We have the following findings: (1)  (2) IVF+DPR$_D$ has similar memory consumption while its effectiveness is much worse than \Framework as shown in Table~\ref{tab:effective}.


% (2) Compared with TkQ and TkQ+DrW, \Framework requires more memory. This is because \Framework pre-generates embeddings for all objects' descriptions in advance while DrW derives the word embeddings during the calculation process. In real scenarios, numerous studies~\cite{li2020compression,micikevicius2017mixed} can be adopted to further reduce the memory cost by embedding compression~\cite{li2020compression} or mix precision techniques~\cite{micikevicius2017mixed}. Therefore, it will not be an obstacle for \Framework's applications. 








% Considering there are numerous studies~\cite{li2020compression,micikevicius2017mixed} to reduce the memory cost by embedding compression or mix precision technique, it will not be an obstacle for \Framework's applications. 

% We acknowledge that there are extensive studies on model compression~\cite{sun2019patient, choudhary2020comprehensive}, inference acceleration~\cite{xin2020deebert, ye2021tr} to reduce the inference time, so it will not be an obstacle for \Framework's applications.



% Furthermore, we acknowledge that there are  extensive studies on model compression~\cite{sun2019patient, choudhary2020comprehensive}, inference acceleration~\cite{xin2020deebert, ye2021tr}, and transfer acceleration~\cite{SpeedTorch}. These efforts have significantly improved the efficiency of inference processes and transfer processes. Therefore, we believe that these aspects will not be a bottleneck in our approach.


\begin{figure*}[!t]
\centering
\subcaptionbox{Beijing\label{fig:exp-robeta}}{
\includegraphics[width=0.9\textwidth]{fig/beijing_tradeoff_roberta.pdf}
}
\subcaptionbox{Beijing\label{fig:exp-linear}}{
\includegraphics[width=0.9\textwidth]{fig/beijing_tradeoff_linear.pdf}
}
\caption{\revision{The effectiveness-efficiency trade-off results for different relevance models (upper and right is better).}}
\label{fig:exp-generalization}
\end{figure*}

\subsection{\revision{Generalization Study of the Proposed Index (RQ3)}}
\noindent\revision{\textbf{Generalization Study.} We explore the applicability of our proposed index to other relevance models designed for embedding based spatial keyword queries. Specifically, we introduce two variants of our relevance model: LIST-R$^{Roberta}$ and LIST-R$^{Linear}$. Specifically, in LIST-R$^{Roberta}$, the BERT model in the dual-encoder module is replaced by another pre-trained language model RoBERTa\footnote{\url{https://huggingface.co/clue/roberta_chinese_base}}~\cite{wolf2019huggingface}. In LIST-R$^{Linear}$, the learned spatial relevance module is replaced with the linear function of distance. We train the two baselines on the Beijing dataset and use them to generate embeddings in advance. We then use our proposed index to build an index on these embeddings and compare it with existing index baselines. The comparison of our proposed index with the baseline indexes is shown in Figure~\ref{fig:exp-generalization}. The experimental results demonstrate that our proposed index maintains a similar advantage over baseline indexes when applied to other relevance models. %validating the superiority of our proposed index across different relevance models.
}



\subsection{Scalibility Study (RQ4)}
\label{sec:exp-scalibility}
\noindent\textbf{Scalability Study.} We evaluate the scalability of \Framework and the proposed relevance model \Framework-R. We supplement the Geo-Glue dataset with new POIs crawled from Open Street Maps in Hangzhou. Since there is no ground-truth data for the relevance between the newly crawled POIs and the existing queries, we only report the efficiency of our proposed retriever \Framework and our relevance model \Framework-R. For the newly acquired POIs, we utilize the trained dual-encoder module and index to partition them into distinct clusters. We report the runtime of \Framework and \Framework-R on Figure~\ref{fig:scalibility}.
% , where the starting point is at 2.8M since the original dataset comprises 2.8M objects. 
We observe that, as the number of objects increases, the runtime of \Framework and \Framework-R scales %efficiently. 
linearly. 
\begin{figure}[!hbtp]
\centering
\subcaptionbox{\Framework-R\label{fig:scalibilty-LISR-R}}{
\includegraphics[width=0.45\columnwidth]{fig/scalibility-LIST-R.pdf}
}
% \hspace{0.02\columnwidth} % 增加一个小的水平间距
\subcaptionbox{\Framework\label{fig:scalibilty-LIST}}{
\includegraphics[width=0.45\columnwidth]{fig/scalibility-LIST.pdf}
}
\caption{Scalability study on the Geo-Glue dataset.}
\label{fig:scalibility}
\end{figure}

%We also measure the training time per epoch of our relevance model and our index on the Beijing dataset, denoted by \Framework-R and \Framework, respectively, varying the size of the training data in the same manner described above. The experimental results are shown in Figure~\ref{fig:percentage_poi_train_time} while other datasets display the same trend. We observe that the training time of \Framework-R and \Framework appears to be linear to the size of the training data, aligning with our complexity analysis.

% \vspace{-1em}

% {\color{red}
%\noindent\textbf{Performance on New Queries and POIs.} Notably, Figure~\ref{fig:percentage_poi_effectiveness} also demonstrates the capabilities of \Framework-R and \Framework in handling new POIs and queries within the same city. This is achieved by abandoning a subset of POIs and their corresponding relevant queries during training and then testing on the full set of POIs to avoid data linkage, which is detailed in the last paragraph. As shown in Figure~\ref{fig:percentage_poi_effectiveness}, \Framework and \Framework-R remain effective in handling new pois and queries.

% }

\subsection{Ablation Studies (RQ4)}
\label{sec:exp-ablation}


% We exclude IVFPQ from this experiment as it is a hybrid index as stated in Section~\ref{sec:exp-setup}, which makes it an unfair comparison.

% \noindent\textbf{Index Study.} To validate the contribution of our proposed index to the overall effectiveness, we compare it with other baseline indexes, including TkQ, IVF, LSH, and HNSW on the Geo-Glue dataset. 
% %We exclude IVFPQ from this experiment as it is a hybrid index as stated in Section~\ref{sec:exp-setup}, which makes it an unfair comparison. 
% We employ each index to retrieve objects and then use our proposed relevance model to rerank these objects. %The default settings are used. 
% %remain consistent with the default ones. 
% The results are reported in Table~\ref{tab:index-effective}, where all baselines are denoted as Index+\Framework-R and use their default hyperparameter settings. We observe that (1) Compared with the IVF+\Framework-R, which has comparative querying speed with \Framework (Table~\ref{tab:runtime}), \Framework obtains a 52.33\% improvement on the recall@10 metric and 46.84\% improvement on the NDCG@1. (2) Our proposed index consistently outperforms other index baselines and delivers at least an order of magnitude faster querying speed. The runtime of Index+\Framework-R is close to the runtime of Index+DPR$_D$, as reported in Table~\ref{tab:runtime}. 


% \begin{table}[h]
%     \centering
%     % \vspace{-0.5em}
%     \caption{Index ablation study on the Geo-Glue dataset.}
%     % \vspace{-0.5em}
%     \label{tab:index-effective}
%     % \small 
%     \renewcommand{\arraystretch}{1.5} % 控制行高
%     \setlength{\arrayrulewidth}{0.5pt}
%     \begin{tabularx}{0.5\textwidth}{>{\centering}m{2.5cm}*{4}{X}}
%         \toprule[1pt]
%         % \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{Geo-Glue}} \\
%         % \cmidrule(lr){2-5} 
%         &\multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} \\
        
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
%         & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1}  \\
%         \midrule[1pt]
%         TkQ+\Framework-R & {0.7890} & {0.7585} & {0.6517} & {0.5639}   \\   
%         IVF+\Framework-R & 0.5381 & 0.5192 & 0.4671 & 0.3960  \\ 
%         LSH+\Framework-R & 0.7665 & 0.7381 &  0.6378 &  0.5555 \\ 
%         HNSW+\Framework-R & 0.7527 & 0.7231 &  0.6219 &  0.5390 \\
%         % IVFPQ+\Framework-R & 0.7990 & 0.7686 & 0.6617 & 0.5739  \\   
%         \midrule
%         \textbf{\Framework} & \textbf{0.8250} & \textbf{0.7909} & \textbf{0.6747} &\textbf{0.5815} \\
%         \bottomrule[1pt]
%     \end{tabularx}
%     % \vspace*{-1em}
% \end{table}






\noindent\textbf{Cluster Quality Study.} To illustrate the quality of produced clusters by our index, we conduct a comparison study. We use the proposed relevance model to generate embeddings and then employ our index (denoted as \Framework-I) and IVF index to produce clusters separately. We present the cluster results of $IF(C)$ and $P(C)$ in Table~\ref{tab:index_ablation_efficiency}, which shows that our index achieves much higher precision and obtains comparative imbalance factors compared with IVF index. %and the cluster reassignment strategy improves $P(C)$ while marginally increasing $IF(C)$. }

% {\color{blue} To illustrate the impact of the cluster reassignment strategy, we show the cluster results of our solution without this strategy, denoted as \Framework (wo) in Table~\ref{tab:index_ablation_efficiency}. Experiment results demonstrate that this strategy substantially improves $P(C)$ while marginally increasing $IF(C)$ on the Beijing dataset. By adjusting the hyperparameter $\lambda$, the threshold value of this strategy, we can manage the trade-off between $P(C)$ and $IF(C)$ to meet different needs.} 

% We also demonstrate the capbili

% The results are shown in. Our index achieves higher precision scores $P$(C) than the IVF index, which suggests the benefit of our strategy of learning to cluster and pseudo-label generation method. For the imbalance factor \text{IF}(C), the index obtains comparative performance as the commonly used K-means, which implies the relatively even distribution of the learned clusters. 

% compare the cluster results of our index, , with  technique in IVF since IVF is the most efficient approach in the experiments. Both methods are built upon the embeddings generated by our proposed model. We exclude the cluster reassignment strategy for fair comparisons. 

\begin{table}[h]
    % \vspace*{-0.5em}
    \centering
    \caption{Comparison of the quality of clusters.}
    % \vspace*{-0.5em}
    \label{tab:index_ablation_efficiency}
    % \small
    \renewcommand{\arraystretch}{1.5} % 控制行高
    \setlength{\arrayrulewidth}{0.45pt}
    \begin{tabularx}{0.5\textwidth}{>{\centering}m{2cm}*{2}{X}*{2}{X}}
        \toprule[1pt]
        \multirow{2}{*}{} & \multicolumn{2}{c}{\textbf{Beijing}} & \multicolumn{2}{c} {\textbf{Shanghai}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & \textbf{\text{IF}(C)} & \textbf{$P$(C)} & \textbf{\text{IF}(C)} & \textbf{$P$(C)} \\
        \midrule[1pt]
        % IR-Tree+\Model & 0.6518 & 0.6311 & 0.5314 & 0.4643 & 0.7168 & 0.6877 & 0.5634 & 0.4746 \\
        % % IVF$^{2k}$+\Model & 0.6304 & 0.5929 & 0.5507 & 0.4267 & 0.4061 & 0.3562 & 0.6388 & 0.6156 & 0.5866 & 0.4783 & 0.4606 & 0.4034 \\ 
        IVF & 1.31 & 0.6774 & 1.33 & 0.6418 \\     
        % \Framework (wo) & 1.34 & 0.8668 &1.31 &0.8331  \\
        \Framework-I & 1.49 & 0.8907 & 1.43 & 0.8382 \\
        \bottomrule[1pt]
    \end{tabularx}
    % \vspace*{-1em}
\end{table}
\noindent\textbf{Pesudo-Label Study.} As discussed in Section~\ref{sec:index}, the parameter $\text{neg}_{\text{start}}$ affects the difficulty level of pseudo-negative labels, which then impacts the effectiveness and efficiency of our index. To investigate the impacts of the pseudo-negative labels, we vary the hyperparameter $\text{neg}_{\text{start}}$ from 40,000, 50,000, 60,000, and 70,000, to 80,000 on the Beijing and Shanghai datasets. We illustrate the metrics $P(C)$ and $\text{IF}(C)$ of produced clusters in Figure~\ref{fig:negstart}. Notably, as $\text{neg}_{\text{start}}$ increases, both $IF(C)$ and $P(C)$ tend to increase. An increased $IF(C)$ suggests a more concentrated distribution of objects, while an increased $P(C)$ indicates improved accuracy in the retrieval results. The experiment results indicate that the choice of $\text{neg}_{\text{start}}$ leads to a trade-off between effectiveness and efficiency, which can be set flexibly in real-world applications.
\begin{figure}[h]
\begin{center}
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/tradeoff_neg_start_if.pdf}
    \caption{The impact over $IF(C)$}
    \label{fig:negstart-if}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/tradeoff_neg_start_precision.pdf}
    \caption{The impact over $P(C)$}
    \label{fig:negstart-pre}
\end{subfigure}
\caption{The impact of neg$_\text{start}$ over the cluster quality.}
\label{fig:negstart}
\end{center}
\end{figure}


% Figure~\ref{fig:negstart-if} illustrates the impact of neg$_\text{start}$ over the imbalance factor $IF(C)$; Figure~\ref{fig:negstart-pre} shows the the impact of neg$_\text{start}$ over the precision $P(C)$.

\noindent\textbf{Spatial Learning Study.} 
%One key component in the relevance model is 
To evaluate the learning-based spatial relevance module, 
%. To perform a comparison study, 
we consider the following baseline: (1) {\Framework-R+$S_{in}$} that replaces the learning-based spatial relevance module with $S_{in}$ for training, where $S_{in}$ = 1 - $SDist(q.loc,o.loc)$; and (2) \Framework-R+$\alpha*S_{in}^{\beta}$ which substitutes the spatial relevance module with a learnable exponential function. $\alpha$ and $\beta$ are two learnable parameters and are processed to ensure non-negative. Table~\ref{tab:ablation} presents the experimental results obtained by conducting a brute-force search on the Beijing dataset using the trained models. Notably, \Framework-R outperforms \Framework-R+$S_{in}$ in all metrics. Interestingly, the first variant outperforms the second variant, which suggests that without careful design, a
learnable function may be outperformed by a simple approach.


% We further illustrate our learned spatial relevance module in Figure~\ref{fig:beijing_dsr}, which is denoted by LSR, to compare with the widely used spatial relevance method $S_{in}$=1-$SDist(q.loc,o.loc)$. Instead of the linear relationships, our \dsr exhibits a sharp increase when $SDist(q.loc,o.loc)$ is close to 0. This finding is consistent with the data observation in Section~\ref{sec:motivations}. 

\begin{table}[!htbp]
% \vspace*{-0.5em}
  \centering
  \caption{Ablation study of spatial relevance module and weight learning via brute-force search on the Beijing dataset.}
  % \vspace*{-0.5em}
  \label{tab:ablation}
  \renewcommand{\arraystretch}{1.5} % 控制行高
  \setlength{\arrayrulewidth}{0.5pt}
  % \small
  \begin{tabularx}{0.5\textwidth}{>{\centering}m{2.5cm}*{4}{X}}
    \toprule[1pt]
    \multirow{2}{*}{} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{NDCG}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & \textbf{@20} & \textbf{@10} & \textbf{@5} & \textbf{@1}\\
    \midrule[1pt]
    \Framework-R + $S_{in}$  & 0.7526 & 0.7087 & 0.5255 & 0.4271 \\
    \Framework-R + $\alpha *S_{in}^{\beta}$ &0.5308 &0.4532 &0.3130 &0.2411 \\
    \Framework-R + ADrW & 0.7925 & 0.7414 & 0.5832 & 0.4792 \\
    \midrule
    \textbf{\Framework-R} & \textbf{0.8156} & \textbf{0.7545} & \textbf{0.5913} & \textbf{0.4989} \\
    \bottomrule[1pt]
  \end{tabularx}
  % \vspace{-0.5em}
\end{table}
\noindent\textbf{Weight Learning Study.} We conduct a comparison experiment between our weight learning module and the attention mechanism proposed by DrW~\cite{liu2023effectiveness} (denoted as ADrW). Table~\ref{tab:ablation} reports the results obtained by conducting a brute-force search on the Beijing dataset using the trained relevance models. Here, \Framework-R represents our weight learning mechanism, while \Framework-R+ADrW denotes replacing it with the ADrW for training. The results indicate that our weight learning mechanism surpasses the latest ADrW mechanism.



% % \subsection{Effect of Training Dataset Size (RQ5)}
% %This suggests that \Framework and \Framework-R are suitable for applications with large datasets.
% \noindent\textbf{Effect of Training Dataset Size on Effectiveness.} %To examine the robustness of \Framework, proposed relevance model \Framework-R, and proposed index, 
% We investigate the impact of training dataset size over \Framework and \Framework-R. Specifically, we exclude a certain percentage of objects along with their corresponding records during the training and validation process. During testing, we use the complete test dataset. This approach avoids the issue of data leakage. We vary the percentage of objects from 30\%, 50\%, 80\% to 100\%. We only present the results for NDCG@1 on the Beijing dataset, as the remaining metrics and datasets have similar results. The results are shown in Figure~\ref{fig:percentage_poi_effectiveness}. \Framework-R uses brute-force search with the relevance model, while \Framework utilizes our proposed index for retrieval. The performance gap between them is consistently small, which underscores the capability of our index to boost retrieval speed without sacrificing effectiveness. 
% %{\color{red} Overall, the efficiency of our index and the retrieval framework \Framework~will not be affected by the training dataset size.}
% \begin{figure}[h]
% % \vspace*{-1em}
% \begin{center}
% \subfigure[\centering {The Impact over Effectiveness}]{
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/robust_plot_ndcg_beijing.pdf}
% }
% \label{fig:percentage_poi_effectiveness}
% }
% % \vspace*{-1em}
% \subfigure[\centering {The Impact over Training time}]{
% \label{fig:shanghai_ndcg}
% % \raisebox{-1.5em}
% {\includegraphics[width=0.45\columnwidth]{fig/robust_plot_traintime.pdf}}
% \label{fig:percentage_poi_train_time}
% }
% % \vspace*{-1em}
% \caption{The impact of training dataset size over effectiveness and training time on the Beijing dataset.
% %over effectiveness and training time.
% }
% %\caption{Figure~\ref{fig:percentage_poi_effectiveness} illustrates the effectiveness of \Framework and its two components as the size of the training data changes. Figure~\ref{fig:percentage_poi_train_time} demonstrates the training time of \Framework and its index as the size of the training data changes.}
% % \vspace*{-1.5em}
% \label{fig:percentage_poi}
% \end{center}
% \end{figure}

% In addition, even with low training percentages (e.g., 0.3), our proposed method maintains satisfactory effectiveness, demonstrating its ability to learn from limited data and adapt to new queries. 

% \noindent\textbf{Effect of Training Dataset Size on Training Time.} 
% We also measure the training time per epoch of \Framework-R and \Framework on the Beijing dataset by varying the size of the training data in the same manner, and the results are shown in Figure~\ref{fig:percentage_poi_train_time}. Other datasets exhibit similar trends. We observe that the training time of \Framework-R and \Framework appears to be linear to the size of the training data, aligning with our complexity analysis.

\noindent{\textbf{Effect of Training Dataset Size on Effectiveness.} We investigate the impact of training dataset size over \Framework and \Framework-R. Specifically, we exclude a certain percentage of objects along with their corresponding records during the training and validation process. During testing, we use the complete test dataset. This approach avoids the issue of data leakage. We vary the percentage of objects from 30\%, 50\%, 80\% to 100\%. \revision{We present the results for NDCG@1 and Recall@10 on the Geo-Glue dataset using default hyperparameters, and similar results are observed for the remaining metrics and datasets.} The results are shown in Figure~\ref{fig:percentage_poi}. \Framework-R uses brute-force search with the relevance model and \Framework utilizes our proposed index for retrieval. The performance gap between them is consistently small, which underscores the capability of our index to boost retrieval speed without sacrificing effectiveness. Additionally, even with low training percentages (e.g., 0.3), our proposed method maintains satisfactory effectiveness, demonstrating its ability to learn from limited data and adapt to new queries.

\noindent\textbf{Effect of Training Dataset Size on Training Time.} We also measure the training time per epoch of \Framework-R and \Framework on \revision{the Geo-Glue dataset} by varying the size of the training data in the same manner stated in the last paragraph, and the results are shown in Figure~\ref{fig:training_time}. Other datasets exhibit similar trends. We observe that the training time of \Framework-R and \Framework appears to be linear to the size of the training data, aligning with our complexity analysis.







\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\columnwidth]{fig/robust_plot_traintime_model.pdf}
\includegraphics[width=0.45\columnwidth]{fig/robust_plot_traintime_index.pdf}
\caption{The impact of training dataset size on training time for the Geo-Glue dataset.}
\label{fig:training_time}
\end{center}
\end{figure}



\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\columnwidth]{fig/robust_plot_ndcg_geoglue.pdf}
\includegraphics[width=0.45\columnwidth]{fig/robust_plot_recall_geoglue.pdf}
\caption{\revision{The impact of training dataset size on effectiveness on the Geo-Glue dataset.}}
\label{fig:percentage_poi}
\end{center}
\end{figure}


% \begin{figure}[h]
% \begin{center}
% \begin{subfigure}[b]{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/robust_plot_ndcg_geoglue.pdf}
%     \caption{}
%     \label{fig:percentage_poi_ndcg}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/robust_plot_recall_geoglue.pdf}
%     \caption{}
%     \label{fig:percentage_poi_recall}
% \end{subfigure}
% \caption{\revision{The impact of training dataset size on effectiveness on the Geo-Glue dataset.}}
% \label{fig:percentage_poi}
% \end{center}
% \end{figure}

\noindent{\textbf{\revision{Effect of Training Sample Selection on Effectiveness.}} \revision{To investigate the impact of training sample selection on effectiveness, we select different 50\% subsets from the Geo-Glue training dataset for training and then compare their effectiveness to demonstrate the influence of training sample choice. Since the random selection is determined by a random seed, we use different seeds (e.g., 1, 2, 3, 4) to ensure that each selection of training samples is different. The experimental results on the Geo-Glue dataset are presented in Figure~\ref{fig:train_sensitivity}, where we only report the results for NDCG@1, and the other metrics are similar. The results show that \Framework and \Framework-R produce similar results across different training samples, demonstrating that our solution is robust to variations in training sample selection.}


\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/train_data_sensitivity_plot_ndcg_geoglue.pdf}
    \caption{}
    \label{fig:train_sensitivity_ndcg}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/train_data_sensitivity_plot_recall_geoglue.pdf}
    \caption{}
    \label{fig:train_sensitivity_recall}
\end{subfigure}
\caption{The impact of training sample selection on effectiveness for the Geo-Glue dataset.}
\label{fig:train_sensitivity}
\end{figure}


% \begin{table}[h]
%     \centering
%      \caption{\revision{Ablation study on training sample selection.}}
%     \label{tab:ablation_train_sample}
%     \renewcommand{\arraystretch}{1.5} % 控制行高
%     \setlength{\arrayrulewidth}{0.5pt}
%     % \small
%     \begin{tabularx}{0.45\textwidth}{>{\centering}m{1.5cm}*{4}{X}}
%     \toprule[1pt]
%     Seed & 0 & 1 & 2 & 3 \\
%     \midrule[1pt]
%     \Framework-R & 0.5606 & 0.5714 & 0.5412 & 0.5565\\
%     \Framework & 0.5488 & 0.5623 & 0.5284 & 0.5423 \\  
%     \bottomrule[1pt]
%   \end{tabularx}
% \end{table}

% \noindent{\textbf{\revision{Evaluating Performance with Low Frequency Descriptors.}} \revision{To investigate the performance of \Framework and \Framework-R in handling POIs with unique or low-frequency descriptors, such as 'halal' or 'vegan', which are more distinctive than common descriptors like 'pizza' or 'pasta', we investigate whether the frequency of object description terms affects the performance of \Framework and \Framework-R on the geo-glue dataset. Specifically, we calculate the frequency of each term and identify POIs containing low-frequency terms, along with their corresponding ground-truth labels. The frequency of object descriptors in the geo-glue dataset ranges from 1 to 962,652. We then select POIs containing terms that appear at most $freq$ times, with $freq$ set to 1, 10, 100, 1,000, and 10,000, and evaluate \Framework and \Framework-R on these subsets to demonstrate their capability in handling POIs with low-frequency descriptions. The experimental results on the geo-glue dataset are shown in Figure~\ref{fig:low_frequency}, where we only report the results for Recall@10 and NDCG@1, as other metrics show similar trends. The results show that \Framework and \Framework-R maintain similar performance for both extremely low-frequency and relatively high-frequency POIs. This demonstrates the robustness of our proposed method.} 

% \begin{figure}[!htbp]
% \centering
% \begin{subfigure}[b]{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/low_frequency_ndcg.pdf}
%     \caption{}
%     \label{fig:low_frequency_ndcg}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/low_frequency_recall.pdf}
%     \caption{}
%     \label{fig:low_frequency_recall}
% \end{subfigure}
% \caption{\revision{%Performance on POIs with 
% Results of Low-Frequency Descriptors.}}
% \label{fig:low_frequency}
% \end{figure}



\begin{figure}[!htbp]
\centering
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/low_frequency_query_ndcg.pdf}
    \caption{}
    \label{fig:low_frequency_ndcg}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/low_frequency_query_recall.pdf}
    \caption{}
    \label{fig:low_frequency_recall}
\end{subfigure}
\caption{\revision{%Performance on POIs with 
Results of Low-Frequency Descriptors.}}
\label{fig:low_frequency_query}
\end{figure}
\noindent{\textbf{\revision{Evaluating Queries Containing Keywords of Low Frequency.}} \revision{To investigate the capability of \Framework and \Framework-R in handling unique or low-frequency keywords, such as 'halal' or 'vegan', which are more distinctive than common keywords like 'pizza' or 'pasta', we investigate whether the frequency of query keywords affects the performance of \Framework and \Framework-R on the geo-glue dataset. Specifically, we calculate the frequency of each keyword and identify queries containing low-frequency keywords, along with their corresponding ground-truth labels. The frequency of query keywords in the geo-glue dataset ranges from 1 to 3,891. %We then select queries containing keywords that appear at most $freq$ times, with $freq$ set to 1, 10, 100, and 1,000, which contains 4108, 15892, 19930, 19991 queries seperately, and evaluate \Framework and \Framework-R on these subsets to demonstrate their capability in handling low-frequency keywords. \
We select queries containing keywords that appear at most $freq$ times, with $freq$ set to 1, 10, 100, and 1,000, resulting in subsets of test queries consisting of 4,108, 15,892, 19,930, and 19,991 queries, respectively. We then evaluate \Framework and \Framework-R on these subsets to demonstrate their capability in handling queries containing low-frequency keywords. The experimental results on the geo-glue dataset are shown in Figure~\ref{fig:low_frequency_query}, where we only report the results for Recall@10 and NDCG@1, as similar trends are observed on other metrics. The results show that \Framework and \Framework-R maintain performance for queries containing keywords of low-frequency. 
%This demonstrates the robustness of our proposed method.
} 


==> framework.tex <==
% \vspace*{-1em}
\section{Proposed Retriever (\Framework)}
\label{sec:LIST}
% \vspace*{-0.5em}
\begin{figure}[t]
%\vspace*{-0.5em}
\centering
\includegraphics[width=0.45\textwidth]{fig/framework.pdf}
% \vspace*{-0.5em}
\caption{The three phases of our retriever \Framework: the training, indexing, and query phase. %\Framework consists of a 
The relevance model is shown in yellow and the index is shown in green.}
% \vspace*{-2em}
\label{fig:framework}
\end{figure}

% \vspace*{-0.5em}
\subsection{Overview}
\label{sec:overview}
\revision{\Framework is featured with a relevance model and a %novel 
machine learning based ANNS index. Notably, our proposed index is applicable to any other relevance model developed for embedding based spatial keyword queries.} % \Framework is featured with a new relevance model and a novel machine learning based ANNS index. Notably, our proposed index is also applicable to any other textual relevance model that transforms query keywords and object text descriptions into two separate embeddings.

The workflow of \Framework is summarized in Figure~\ref{fig:framework}, which has three phases: training, indexing, and query phase. During the training phase, we first train the relevance model, and then train our index. During the indexing phase, each object is partitioned into one cluster. During the query phase, the trained index routes each query to either a single cluster or a subset of clusters that have the highest probabilities. Within these clusters, \Framework returns $k$ objects with the highest scores ranked by the trained relevance model as the query result.

%Note that our index is not limited to our proposed relevance model, and can also be applied for other embedding-based spatio-textual relevance models.

%\noindent\textbf{Challenges.} The first challenge is how to train an effective relevance model that can capture both textual and spatial relevance. To address this challenge, we propose a new relevance model that comprises a textual relevance module, a learning-based spatial relevance module, and an adaptive weight learning mechanism.

%The second challenge is how to build an index to support both spatial relevance and dense vectors based textual relevance. To address this challenge, 
%inspired by the inverted file index~\cite{jegouProductQuantizationNearest2011}, 
%we propose a machine learning  based index, which extends the learning-to-cluster approach to cluster relevant objects and queries together while separating irrelevant objects and queries. Existing learning-to-cluster techniques~\cite{Hsu16_KCL,Hsu18_L2C} depend on the labels of images for training, which is absent in geo-textual data. Moreover, when the number of clusters exceeds the number of image classes, the existing technique tends to partition images to a few large clusters~\cite{Hsu16_KCL}, which will hurt the efficiency. To tackle the two issues, we propose a novel pseudo-label generation method, which provides informative labels to enable the index to capture both spatial and textual information.  To further improve the cluster's quality, we also propose a non-trivial cluster reassignment strategy. 


% To address this challenge, we leverage the Learning-to-Cluster approach~\cite{Hsu16_KCL,Hsu18_L2C}, aiming to cluster relevant spatial keyword queries and geo-textual objects together while separating irrelevant ones. However, existing techniques~\cite{Hsu16_KCL,Hsu18_L2C} depend on the ground-truth labels of images to provide similar or dis-similar labels during training, which is absent in geo-textual data. Besides, when the cluster number $c$ exceeds the number of image classes, the existing technique tends to partition images to a few large clusters~\cite{Hsu16_KCL}, such highly skewed cluster distribution would hurt the efficiency. To tackle the two issues, we propose a novel pseudo-label generation method, which employs the trained relevance model to produce high-quality pseudo-labels. To further improve the cluster's quality, we propose a non-trivial cluster reassignment strategy after the index's training.




% To automatically learn to balance spatial and textual relevance, we turn to a learning-based approach to cluster geo-textual objects, i.e., Learning to Cluster~\cite{Hsu16_KCL,Hsu18_L2C}. 


% This method employs a multi-perception layer (MLP) to produce a $c$-cluster probability for each image and train the MLP to cluster similar images and differentiate those dis-similar images. However, ground-truth labels of images can be used as similar/dis-similar labels in the training, but such labels are absent in geo-textual data. Besides, when $c$ exceeds the number of image classes, the existing technique tends to partition images to a few large clusters~\cite{Hsu16_KCL}, such highly skewed distribution would hurt the efficiency of our task. To tackle these two challenges~\cite{Hsu16_KCL,Hsu18_L2C}, we propose a novel pseudo-label generation method, which employs the trained relevance model to generate high-quality pseudo-labels. To further improve the cluster's quality, we propose a non-trivial cluster reassignment strategy after the index's training.



% Motivated by the inverted file index~\cite{jegouProductQuantizationNearest2011}, which has been discussed in Section~\ref{sec:related}, we propose a novel learnable inverted file index, which aims to cluster relevant queries and objects together while separating irrelevant ones.


% Recently, a new neural network-based end-to-end clustering framework has been introduced, namely,  This framework utilizes an MLP, called the cluster classifier,  Then it trains the MLP to 


% Instead of using the heuristic algorithm, we leverage the new learning-to-cluster approach, aiming to assign relevant objects and queries into the same cluster. 







% Inspired by them, we explore a novel approach, i.e., learning to cluster for the spatial-textual objects, which has not been studied yet. However, this exploration is non-trivial, as we cannot straightforwardly use the existing techniques for spatial-textual data. Specifically, images have ground-truth labels, which are used as similar/dis-similar labels in the training, but such labels are absent in geo-textual data.  To develop a solution for learning Geo-Textual data to clusters, we must address these obstacles.





% Compared with existing ANNS indices, our proposed index benefits from the ground-truth labels and pseudo-negative labels, providing a better accuracy-efficiency trade-off.


% To answer the \tkskq both effectively and efficiently, we design a novel learnable inverted file retriever for spatial-textual data (\Framework), which consists of two parts: (1) learn an effective relevance model, and (2) train an index for the relevance model.





% uses a dual-encoder-based relevance model to map the object descriptions into a $d$-dimensional dense vector and builds an index for all objects based on the object's vector and location, which we will use for retrieval.
% \vspace{-1em}
% \vspace*{-0.5em}
\subsection{The  Relevance Model}
\label{sec:model}
\noindent\textbf{Textual Relevance Learning.} Inspired by the dual-encoder model's success in document retrieval~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20}, we employ a dual-encoder module to encode query keywords and object description into two separate embeddings, %thereby transform spatial keyword queries into embedding based spatial keyword queries 
and calculate textual relevance by the inner product between the two embeddings. %To our knowledge, this is used in spatial keyword query for the first time. 
Compared with previous relevance models~\cite{liu2023effectiveness} that rely on word embeddings and complex word interaction functions discussed in Section~\ref{sec:related}, %neural networks, 
the dual encoder module is both efficient and effective.%, as discussed in Section~\ref{sec:related}}

%as the object text embeddings can be pre-computed and build an index upon them, while the complex neural networks cannot be pre-calculated until we see the input pair query-object pair, as discussed in Section~\ref{sec:related}}

%offers two advantages: (1) it is more friendly to build an index upon the proposed relevance model as the object text embeddings can be pre-computed and build an index upon them, unlike previous deep models that rely on dozens of word embeddings and the textual relevance between queries and objects cannot be computed until seeing the query-object pair~\cite{liu2023effectiveness}, and (2) it is more efficient to compute textual relevance.} 
%structure to capture the textual relevance between queries and objects. 


The dual-encoder module comprises an object encoder $E_o$ and a query encoder $E_q$, \revision{each of which is a BERT model~\cite{devlin2018bert}.} The encoder takes the textual content of the query or object as input, captures interactions between words by the transformer-based model, and finally utilizes the representation of the [CLS] token as the global semantic representation, which is a $d$-dimensional embedding. This process is formulated as:
\begin{equation}
\begin{aligned}
    o.emb = E_{o}(o.doc; \theta_o), \: o.emb \in \mathbb{R}^{d}, \\
    q.emb = E_{q}(q.doc; \theta_q), \: q.emb \in \mathbb{R}^{d}.     
\end{aligned}
\label{eq:DE}
\end{equation}
where $E_{o}(·; \theta_o)$ denotes the object encoder parameterized with $\theta_o$ and $E_{q}(·; \theta_q)$ denotes the query encoder parameterized with $\theta_q$. Then the text relevance score is calculated by the inner product between the $q.emb$ and $o.emb$,
\begin{equation}
TRel(q.doc,o.doc) = q.emb \cdot o.emb.
\label{eq:textual-relevance}
\end{equation}


{\color{red} }




% As discussed in Section~\ref{sec:data-obs-ana}, existing methods either utilize the conventional bag-of-words models or term interactions-based deep learning methods~\cite{liu2023effectiveness}, which would suffer from effectiveness or efficiency issues. Different from previous studies,  These encoders utilize , to convert textual content into $d$-dimensional real value vectors. During the indexing phase, the object encoder takes as input the textual content of geo-textual objects $o.doc$, converting it to a $d$-dimensional vector $o.emb$. Similarly, during the query phase, the content of query $q.doc$ is converted to $q.emb$ by the query encoder. These two processes 

% where $E_{o}(·; \theta_o)$ denotes the object encoder parameterized with $\theta_o$ and $E_{q}(·; \theta_q)$ denotes the query encoder parameterized with $\theta_q$. The usages of these textual embeddings are two-fold. On one hand, the text relevance score can be calculated by the inner product between the $q.emb$ and $o.emb$, as depicted as follows: 

% On the other hand, these textual embeddings, linked with their respective geo-locations, can be utilized to construct the index of objects, which will be presented in detail in Subsection~\ref{sec:index}.  %for partitioning or routing.

\noindent\textbf{Spatial Relevance Learning.} As discussed in Section~\ref{sec:motivations}, it is essential to develop a more effective spatial relevance module. Therefore, we propose a new learning-based spatial relevance module to learn to estimate spatial relevance.

% To better fit the real-world scenario described in Section~\ref{sec:motivations}, it is essential to assign higher spatial relevance to nearby objects and lower spatial relevance to distant objects. {\color{red} And as mentioned in Section~\ref{sec:intro}, directly employing an exponential function is even less effective. }

%, where $S_{in}=1-SDist(q.loc,o.loc)$ is taken as input. }

%A straightforward approach would be to employ an exponential function. However, our experiments indicate that this method is even less effective compared to the linear function (shown in Section~\ref{sec:exp-ablation}). 

As discovered in Section~\ref{sec:motivations}, the user's geographic preferences for geo-textual objects do not follow a linear pattern. \revision{Here, we consider two features of the %user's geographic 
preference: %for geo-textual objects 
%has two feature: 
(1) it increases as the distance decreases, and (2) it exhibits a stepwise decline as the distance increases. The first feature is straightforward because users tend to visit nearby objects. Then a straightforward solution is to design a monotonically continuous function to learn from query-object positive pairs and predict users' spatial preferences. However, this approach leads to overfitting. For example, if most positive pairs within training dataset are distributed within 1km, the continuous function will learn 1km as a boundary, causing high spatial relevance within 1km but a sharp drop beyond it. Actually, 1.1km is not significantly different from 1km for users. This overfitting results in poor performance due to lack of generalization (as to be shown in Section~\ref{sec:exp-ablation}). To alleviate this issue, we propose the second feature. To explain this stepwise pattern, let us consider a scenario in which a customer wishes to purchase coffee from Starbucks. If the nearest Starbucks is very close, s/he would go and buy coffee. If the nearest Starbucks is a little far, s/he may hesitate and her/his intention of visiting the Starbucks would decrease. If the nearest Starbucks is very far away, s/he would give up this idea. Therefore, this pattern aligns with real-world characteristics and alleviates the overfitting issue as the boundaries are manually based on our knowledge. In summary, the new spatial relevance module is designed to be a learnable monotonically step function.}





Our proposed spatial relevance module takes $S_{in}=1-SDist(q.loc,o.loc)$ as input, consisting of a threshold array $\mathcal{T} \in \mathbb{R}^{t \times 1}$ and a learnable weight array $w_s \in \mathbb{R}^{1 \times t}$. Here, $\mathcal{T}$ stores the threshold values that determine the transition points of the step function, i.e., the value exceeded by $S_{in}$ will trigger an increase of spatial relevance, which is used to ensure that the learned function is a step function. Specifically, $\mathcal{T}$ is structured as $\mathcal{T}[i] = \frac{i}{t}$, where $i \in [0,t]$ and $t$ is a hyperparameter to control the increment of the threshold value. For example, when $t=100$, $\mathcal{T}$ is $[0.0,0.01,\cdots, 0.99,1.0]$. The learnable weight array $w_s$ determines the extent of the increase when the input $S_{in}$ reaches these threshold values, which are learned from the training data and used to estimate the spatial relevance. When the input $S_{in}$ exceeds the value of $\mathcal{T}[i]$, then the spatial relevance increases by $act(w_s[i])$, where $act$ is an activation function to ensure $act(w_s[i])$ remain non-negative. This process ensures that the output $SRel$ exhibits a step increase as the input $S_{in}$ increases. The learned spatial relevance is computed as below: 
%$w_s$ is employed to learn and estimate the spatial relevance. 
%Specifically, $\mathcal{T}$ stores the threshold values that determine the transition points of the step function, i.e., the value exceeded by $S_{in}$ will trigger an increase of spatial relevance. 
%Note that weights in $w_s$ are learned from the training data.  
\begin{equation}
    SRel(q.loc,o.loc) = act(w_{s})  \cdot \mathbb{I}(S_{in} \geq \mathcal{T}[i]),
\label{eq:DSR}
\end{equation}
where $SRel(q.loc,o.loc)$ is the learned spatial relevance. $\mathbb{I} \in \{0,1\}^{t \times 1}$ is an indicator array. $\mathbb{I}[i]=1$ if $S_{in} \geq$ $\mathcal{T}[i]$; otherwise 0. The sum of the step increment is conducted by an inner product between the indicator array $\mathbb{I} \in \{0,1\}^{t \times 1}$ and the learnable weight after activation $act(w_{s}) \in \mathbb{R}^{1 \times t}$.


% Previous studies usually directly employ $1-SDist(q.loc,o.loc)$ as spatial relevance, where $SDist(,)$ denotes the normalized Euclidean distance. Motivated by the findings in Section~\ref{sec:motivations}, 




%The Deep learning-based Spatial Relevance module (\dsr) is designed to learn such a spatial relevance, which takes $1-SDist(q.loc,o.loc)$ as input. 
%If the nearest Starbucks is far away, he abandons this idea. 
%his intent to buy coffee remains unchanged. If the nearest Starbucks is a little far, he hesitates. If the nearest Starbucks is far away, he abandons this idea. 




During the query phase, we extract the weights in $w_{s}$ from the module and store them as an array $\hat{w_{s}}$ for faster inference. $\hat{w_{s}}$ is constructed as $\hat{w_{s}}[i] = \sum\limits_0^{i}act(w_{s}[i])$. When computing the spatial relevance, we get the input $S_{in}$. Since the threshold value grows uniformly by $\frac{1}{t}$, we can determine the number of threshold values exceeded by the input as $\lfloor S_{in}*t \rfloor$, where $\lfloor . \rfloor$ indicates a floor function and is utilized to truncate a real number to an integer. This also corresponds to the sum of the values of weights, which is the spatial relevance score. This process is formulated as:
\begin{equation}
SRel(q.loc,o.loc) = \hat{w_{s}}[\lfloor S_{in}*t\rfloor].
\label{eq:DSR_inference}
\end{equation}
Hence, during the query phase, the time complexity of computing spatial relevance is O(1), which is efficient. 


\noindent\textbf{Adaptive Weight Learning.} The recent study~\cite{liu2023effectiveness} has shown the importance of weight learning in improving ranking effectiveness. To enhance ranking effectiveness, we propose an adaptive weight learning module, which aims to assign adaptive weights to textual and spatial relevance based on the query keywords. \revision{For instance, in the case of detailed query keywords, such as `gas station nearby', giving lower weight to textual relevance better fits the real-world scenario. Since there may be many gas stations nearby, users tend to prefer the closest one. Conversely, in another scenario, such as searching with keywords `Lincoln Memorial in Washington, D.C.', due to the uniqueness of the keyword, giving greater weight to textual relevance can deliver better results.}


%It first employs neural networks to extract textual information from the query's word embeddings and capture spatial information from location embeddings, and then collaboratively learns the optimal weights. However, rather than utilizing embeddings of each word in the query, 
%Here, we utilize the embedding of query keywords $q.emb$, which is obtained by the dual-encoder module, to compute adaptive weights. %In addition, our empirical experiments show that the location embedding technique 
%is not beneficial, which would introduce additional computational costs. 
Hence, we employ a simple yet effective manner that directly utilizes an MLP layer to determine the weights based on the embedding of query keywords $q.emb$, which is formulated as follows:
\begin{equation}
    w_{st} = MLP(q.emb), \: w_{st}\in \mathbb{R}^{1\times 2}.
\label{eq:model_weight}
\end{equation}

%The previous study~\cite{liu2023effectiveness} applies a term interaction module to the query's text to estimate the optimal weights for each query. This is inspired by the document ranking models~\cite{DBLP:journals/corr/abs-1903-06902}, which leverage term embeddings' interactions between queries and documents to identify relevant terms, thereby finding relevant documents for input queries and improving ranking effectiveness. However, it's not very reasonable to directly apply this motivation to weight learning, as the term interaction between words of the query doesn't necessarily result in optimal weights.

%To design a more effective weight learning mechanism, we conduct two experiments to guide the mechanism's design. We divide the train queries in Beijing dataset into two groups: `Short Text' (queries with less than 2 keywords) and `Long Text' (queries with more than 6 keywords). On average, queries have 4.17 keywords. The first experiment is to compare different queries' CDF, as shown in Figure~\ref{fig:cdf_distribution}. `Short Text' has a more sharp CDF compared with `Long Text'. In the second experiment, we determine the optimal text weight $\alpha$ for different queries by adjusting $\alpha$ from 0 to 1 with a footstep of 0.1, where the ranking model is Equation~\ref{eq:TkSKQ_rank} and $TRel(q.doc,o,doc)$ is calculated by BM25~\cite{DBLP:journals/ftir/RobertsonZ09}. As demonstrated in Figure~\ref{fig:optimal_weight_distribution}, `Short Text' has a narrower optimal $\alpha$ distribution compared with `Long Text'. The underlying rationale of the two experiments' results is that longer texts are usually more informative and thus less likely to be impacted by distance, while shorter texts are less informative and thus are more likely to be influenced by distance. This analysis motivates us to design the mechanism based on the volume of information within the query's sentence embedding.

% {\color{blue}
% Based on the above motivation, we aim to design a novel query-driven Information Extraction Mechanism (\iem). However, extracting the volume of information from a sentence embedding remains an unsolved problem. Therefore, we leverage the well-known transformer self-attention mechanism~\cite{devlin2018bert}, which achieves great success in extracting information from long documents. The \iem takes as input $q.emb$. \iem firstly splits $q.emb$ into several subvectors, then uses the transformer attention mechanism to extract information from each subvector and sum up the attention value as depicted below: 

% }

Similar to the Equation~\ref{eq:TkSKQ_rank}, the final relevance score between the query and the object is calculated as:
\begin{equation}
    ST(q,o) = w_{st}\cdot [TRel(q.doc, o.doc), SRel(q.loc,o.loc)]^{T}. 
\label{eq:model_rank}
\end{equation}

\noindent\textbf{Training Strategy.} To train our relevance model, we employ the 
%powerful 
contrastive learning strategy. Given a query $q_i$, the positive (relevant) geo-textual object $o_i^{+}$ is obtained by real-world %click-through 
ground-truth data (detailed in Section~\ref{sec:exp-setup}). As for the negative (irrelevant) geo-textual objects, previous studies of passage retrieval~\cite{DBLP:conf/naacl/QuDLLRZDWW21,renRocketQAv2JointTraining2021} have shown that hard negative objects can improve retrieval performance. Inspired by them, we introduce this mechanism for spatial keyword query, choosing a subset of hard negative objects for training. Specifically, for each training query, we first filter out the positive objects and then use TkQ~\cite{congEfficientRetrievalTopk2009} to retrieve a set of top-ranked objects, which are considered the hard negative set for that query. In each training epoch, we randomly pick $b$ hard negative samples from this set. We optimize the loss function as the negative log-likelihood of the positive object: 

% \gao{why 5000? do we need to give the number?}
% \vspace*{-1em}
\begin{equation}
% \small
% L_{\text{model}} (q_i, o_i^{+}, o_{i,1}^{-}, o_{i,2}^{-}, \cdots, o_{i,b}^{-})= -log \frac{e^{ST(q_i, o_i^{+})}}{e^{ST(q_i, o_i^{+})} + \sum_{j=1}^{b}e^{ST(q_i, o_{i,j}^{-})}}.
% \label{eq:loss}
\begin{split}
    L_{\text{model}} & (q_i, o_i^{+}, o_{i,1}^{-}, o_{i,2}^{-}, \cdots, o_{i,b}^{-}) \\
    & = -log \frac{e^{ST(q_i, o_i^{+})}}{e^{ST(q_i, o_i^{+})} + \sum_{j=1}^{b}e^{ST(q_i, o_{i,j}^{-})}}.
    \label{eq:loss}
\end{split}
\end{equation}
In addition, we also utilize the in-batch negatives strategy~\cite{lin2021inbatch} to further enhance training efficiency.

\noindent\revision{\textbf{Complexity Analysis.} Now we analyze the time %and space 
complexity of the proposed relevance model. Assuming the dimensionality of the embedding is $d$, the total number of objects is $n$, and the embeddings of objects are generated in advance. The time complexity of a brute-force search of our relevance model over the entire dataset is $O(n(d + 2) + d)$. Here, $O(nd)$ represents the time cost of Equation~\ref{eq:textual-relevance}, $O(2n)$ corresponds to the time cost of Equation~\ref{eq:DSR_inference}, and $O(d)$ accounts for the time cost of Equation~\ref{eq:model_weight}.} 

\revision{When compared with other relevance models like DrW~\cite{liu2023effectiveness}, which has a time complexity of $O(nl^q(l^od+k')+l^q(2d^2+d))$, our relevance model exhibits superior efficiency in terms of time complexity. Here, $l^q$ represents the number of words in the query keywords, $l^o$ represents the number of words in the object description, and $k'$ denotes the number of top-k' relevant terms to find in the object description for each query keyword. These hyperparameters, $l^q$, $l^o$, and $k'$, are typically in the dozens. Consequently, DrW is significantly slower than our relevance model.}
%and space complexities.  } 


\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{fig/index.pdf} 
  \caption{The illustration of the index.}
  \label{fig:index}
\end{figure}

\subsection{The Proposed Index}
\label{sec:index}
%As described earlier in Section~\ref{sec:model}, our proposed relevance model can transform spatial keyword queries into embedding based spatial keyword queries. 
In this section, our objective is to develop a new ANNS index that, for each embedding based spatial keyword query, can return a subset of objects that receive high scores from the proposed relevance model for the input query, thereby accelerating the top-k search process. %However, our proposed relevance model requires evaluating both textual and spatial relevance between queries and objects simultaneously, and the weights also vary with the query embedding. This presents a significant challenge in designing such an ANNS index. 

%Despite already having a lightweight and effective spatio-textual relevance model, there is such an ANNS specifically designed for the spatio-textual relevance model. As discussed in Section~\ref{sec:related}, existing ANNS indexes typically reduce the search space by identifying a subset of similar embeddings using heuristic methods. However, as described earlier in Section~\ref{sec:model}, our proposed relevance model requires evaluating both textual and spatial relevance between queries and objects simultaneously, and the weights also vary with the query embedding. This presents a significant challenge in designing a new ANNS index.

To build such an index, %different from the heuristic approaches used by previous ANNS indexes~\cite{jegouProductQuantizationNearest2011,liu2019lsh,DBLP:journals/pvldb/FuXWC19}, 
our proposed index adopts a machine learning based method. Without manually setting the weight between spatial and textual relevance, it learns to cluster relevant queries and objects together while separating the irrelevant ones. Specifically, as illustrated in Figure~\ref{fig:index}, it takes the geo-location and textual embeddings of objects or queries as input and employs a Multi-Layer Perceptron (MLP) to partition objects and route queries into $c$ clusters, and then searches for the top-k relevant objects within the routed cluster. To make the index both effective and efficient, we develop a novel pseudo-negative query-object pair generation method. These pseudo labels combined with the positive (relevant) query-object pairs ensure that relevant queries and objects are partitioned and routed into the same cluster while separating the irrelevant ones, thereby reducing the search space while maintaining effectiveness.


\noindent\textbf{Feature Construction.} 
% To input geo-textual objects and queries into neural networks, we utilize the $(q.loc,q.emb)$ and $(o.loc,o.emb)$ to construct a consistent input representation for both objects and queries. 
%Specifically, our index takes as input a location-linked embedding, denoted as $(loc,emb)$, where the geo-location $loc=\langle lat,lon \rangle$ comprises a latitude and a longitude, and $emb \in \mathbb{R}^d$ is a $d$-dimensional vector converted from $o.doc$ or $q.doc$ by the dual encoder module. Then we construct the input representation as depicted below: 
We utilize geo-location and textual embedding to construct a consistent input representation for both objects and queries, which is illustrated in Figure~\ref{fig:index}. \revision{The textual embedding $emb \in \mathbb{R}^d$ is a $d$-dimensional embedding converted from textual content $o.doc$ or $q.doc$ by the trained dual encoder module, which is typically hunderds, e.g., 768. It is L2 normalized before being input into the neural network.} The geo-location $loc=\langle lat,lon \rangle$ are transformed into the following features $\langle \hat{lat}, \hat{lon} \rangle$ as below:  
\begin{equation}
\hat{lat} = \frac{lat-lat_{min}}{lat_{max}-lat_{min}}, \hat{lon} = \frac{lon-lon_{min}}{lon_{max}-lon_{min}},
\label{eq:normalize}
\end{equation}
where $lat_{min}$ ($lon_{min}$) represents the lowest latitude (longitude) in dataset $D$, $lat_{max}$ ($lon_{min}$) denotes the highest latitude (longitude) in dataset $D$. Then the input representation is formulated as 
\begin{equation}
x = [emb, \hat{lat}, \hat{lon}].
\label{eq:representation}
\end{equation}
Here $x$ is the input feature vector for the cluster classifier, i.e., the MLP. \revision{Since the two feature vectors are normalized independently, they will have a similar impact on the neural network.}%Although several region embedding techniques exist~\cite{paul2021semantic}, we %discover find that this simple approach is sufficiently effective. 

\noindent\textbf{Cluster Classifier.} Our cluster classifier is a lightweight Multi-Perception Layer (MLP). Given $x$ as the input, it produces the $c$-cluster probability distribution, defined as follows:
\begin{equation}
    Prob = Softmax(MLP(x)), \: Prob \in \left[0, 1\right]^{c \times 1},
    \label{eq:L2PO}
\end{equation}
where $c$ is a hyperparameter that indicates the desired number of clusters we aim to obtain, and $Prob$ represents the predicted $c$-cluster probability distribution. The $c$-cluster probability distribution of object $o$ is denoted as $Prob_o$ and that of query $q$ is represented as $Prob_q$. 

Note that the cluster classifier, i.e., the MLP, is shared between queries and objects. This setting allows our index to learn the distribution of both queries and objects, subsequently grouping identified relevant queries and objects into the same cluster (as detailed later).


%The MLP is shared between queries and objects.  

%The cluster classifier actually serves as a relevance classifier, grouping identified relevant queries and objects into the same cluster. 




% Randomly sampling some objects as negative pairwise labels is not advisable as low-quality negative labels will lead to overfitting where every object and query are grouped together (as detailed later).

\noindent\textbf{Pseudo-Label Generation.} To train the cluster classifier, both positive and negative pairwise labels are required. We utilize the ground-truth query-object relevant label (e.g., click-through or human annotation, detailed in Section~\ref{sec:exp-setup})  as the positive pairwise label for training. However, we lack high-quality negative pairwise labels. Randomly selecting negative objects will lead to overfitting and all objects are grouped together (as detailed later). Therefore, we propose a novel pseudo pairwise negative label generation method. 

The relationship between query $q$ and object $o$ is denoted as $s(q,o)$. If $q$ and $o$ are relevant %(e.g., users click the object)
, $s(q,o)=1$; otherwise, $s(q,o)=0$, which are then used as labels for training. We leverage ground-truth positive labels as pairwise positive labels in the training, as shown below: 
\begin{equation}
% \vspace{-1ex}
    \text{pos}_{q} = \{o; o\in D, s(q,o)=1\},
    \label{eq:positive_pool}
    % \vspace{-1ex}
\end{equation} 
where the positive object set of query $q$ is denoted as $\text{pos}_{q}$.

The negative object set $\text{neg}_{q}$ of query $q$ is generated by the relevance model. Given a query $q$, we employ the relevance model to calculate the relevance score for all objects. Then we adaptively select $\text{neg}_{q}$ according to two hyperparameters $neg_{start}$ and $neg_{end}$, as shown below:
\begin{equation}
% \vspace{-1ex}
    \text{neg}_{q} = \text{argsort}_{o \in D} ST(q,o)[neg_{start} : neg_{end}], \; s(q,o)=0,
    \label{eq:negative_pool}
    % \vspace{-1ex}
\end{equation} 
where $ST(q,o)$ is the relevance score between query $q$ and object $o$ produced by the relevance model. Note that positive query-object pairs are excluded as indicated by the filter condition $s(q,o)=0$. %We emprically set $neg_{end}$=$neg_{start}+5,000$. %, so $neg_{start}$ directly controls $\text{neg}_{q}$. 

This adaptive pseudo-negative generation method draws inspiration from hard negative sample strategy~\cite{DBLP:conf/naacl/QuDLLRZDWW21,renRocketQAv2JointTraining2021}. What sets our approach apart from existing studies~\cite{DBLP:conf/naacl/QuDLLRZDWW21,renRocketQAv2JointTraining2021} is that we employ an adaptive manner to select hard negative samples, thereby controlling the difficulty level of the generated negative samples. This adjustment strikes the trade-off between the effectiveness and efficiency. %of our indexing method. 

Decreasing $neg_{start}$ leads to a set of harder negative objects being chosen to train the model. Consequently, the classifier is more effective in distinguishing between positive objects and hard negative objects, which facilitates the clustering of relevant queries and objects, while effectively segregating the irrelevant ones. Empirically, under this setting, only the very relevant queries and objects are grouped into the same cluster. The reduced number of objects within a query's cluster leads to higher efficiency. In contrast, when using a large $neg_{start}$, the index can not learn useful information, leading to a scenario where all objects tend to be clustered together.

On the other hand, when our index is trained on a set of harder negative objects, it might also exclude some positive ones and reduce its effectiveness. Thus, the choice of $neg_{start}$ strikes a trade-off between effectiveness and efficiency. This alleviates the lack of negative label issue and the skewed cluster distribution issue of existing techniques~\cite{Hsu16_KCL,Hsu18_L2C}.

% This adaptive pseudo-negative generation method is inspired by the hard negative sample strategy~\cite{DBLP:conf/naacl/QuDLLRZDWW21,renRocketQAv2JointTraining2021}, which have been used in Section~\ref{sec:model}. Different from existing studies, we employ an adaptive manner to control the level of difficulty for the generated negative samples, which aims to balance the effectiveness and efficiency of the index. On one hand, decreasing $neg_{start}$ leads to a set of harder negative objects being chosen to train the model. Then the classifier is more effective in distinguishing between positive objects and hard negative objects, subsequently clustering identified negative objects and queries into different clusters. Empirically, under this setting, only the very relevant queries and objects are grouped together in the same cluster, resulting in higher efficiency since less number of objects will be considered. On the other hand, when our index is trained on a harder set of negative objects, it might also exclude some positive ones, which reduces the recall of the answer. This is because the part of ground-truth objects and the given query would be mistakenly classified into distinct clusters. Thus, the choice of $neg_{start}$ strikes a trade-off between effectiveness and efficiency. This approach alleviates the lack of negative label issue and the skewed cluster distribution issue of existing techniques~\cite{Hsu16_KCL,Hsu18_L2C}.


% which provides more flexibility. 

  

% which employs a trained relevance model to rank the entire dataset for each query $q$, then the top-k negative objects are used as hard negative samples to train a more effective relevance model. 

  

% As these hard negative samples are harder to distinguish, a more effective model can be trained. 

 

% While spatial-textual objects lack labels, making existing techniques~\cite{Hsu16_KCL,Hsu18_L2C} unsuitable, we utilize positive and negative pairs of $\langle q, o \rangle$ as pseudo-labels for training. 

%Empirically, when we aim for high efficiency, we decrease $neg_{start}$. Since training the index with a harder negative object set ensures that only more relevant queries and objects are grouped together in the same cluster. 
  
%This is due to our index utilizing a lightweight model like MLP, which inherently has limited capability. 





%The reason for using our proposed ranking model to select the hard negative sample set instead of other methods such as BM25~\cite{DBLP:journals/ftir/RobertsonZ09} is that it enables better integration between the index and the ranking model. Consider an ideal scenario: if our index perfectly learns the characteristics of the hard negative object set, then it filters out all simpler negative objects and remains harder objects in the same cluster of the query. The negative object set generated by other methods still results in effectiveness degradation due to the ranking model discrepancies, whereas our method leads to no effectiveness degradation.

% Although the spatial-textual objects do not have labels, which means the existing techniques~\cite{Hsu16_KCL,Hsu18_L2C} cannot be employed, we use the positive and negative pairs of $\langle q, o \rangle$ as the pseudo-labels for training. This pseudo-label generation method solves the lack of label challenge and the choice of $neg_{start}$ solves the object concentration issue.

%This pseudo-label generation method solves the lack of label challenge. In addition, decreasing $neg_{start}$ not only results in a decreased number of objects clustered into the same cluster of the query but also reduced queries within the same cluster. This is because the MLP is shared between objects and queries, then only more similar queries are grouped into the same cluster. This indicates that decreasing $neg_{start}$ leads to a more evenly distribution of queries, which helps to alleviate the object concentration issue mentioned before. 


\noindent\textbf{Training Strategy.} Based on the hard negative objects and positive objects provided above, we employ the MCL loss function~\cite{Hsu19_MCL} to train the MLP, as described below: 
% \vspace{-1em}
\begin{equation}
% \small
% L_{\text{Index}}(q_i, o_i^{+}, o_{i,1}^{-}, o_{i,2}^{-}, \cdots, o_{i,m}^{-})= log(\hat{s}(q_i, o_i^{+})) + \sum\limits_{j=1}^{m} log(1-\hat{s}(q_i,o_{i,j}^{-})),
\begin{split}
L_{\text{Index}} & (q_i, o_i^{+}, o_{i,1}^{-}, o_{i,2}^{-}, \cdots, o_{i,m}^{-})\\
    & = log(\hat{s}(q_i, o_i^{+})) + \sum\limits_{j=1}^{m} log(1-\hat{s}(q_i,o_{i,j}^{-})),
\end{split}
\label{eq:MCL}
\end{equation}
where $\hat{s}(q_i,o_j) = Prob^{T}_{q_i}\cdot Prob_{o_j}$, $o_i^{+} \in \text{pos}_q$ and $o_{i,j}^{-} \in \text{neg}_q$. Typically, we randomly select one positive object $o_i^{+}$ from the positive object set $\text{pos}_q$ and $m$ negative objects from the negative object set $\text{neg}_q$ in each training epoch. 

% for training purpose.

As described earlier, the MLP is shared between queries and objects. Through this training process, for positive query-object pairs, their $Prob_o$ and $Prob_q$  will have a similar distribution. Thereby, relevant pairs of query and object are more likely to be grouped into the same cluster while the irrelevant pairs are grouped into distinct clusters. For example, as illustrated in Figure~\ref{fig:index}, the object $o_4$ and query $q_2$ form a positive query-object pair, and they are expected to be grouped into the same cluster $C_2$.

%As we aim at grouping the relevant pairs of query and object into the same cluster while the irrelevant pairs are into distinct clusters, the queries and objects are jointly incorporated. This is because the MLP is shared between objects and queries. In this manner, the complex relationships between queries and objects can be well learned in the process of index construction. Figure~\ref{fig:index} also demonstrates this process, where relevant pairs share similar output and irrelevant ones have different output.


\noindent\textbf{Learning to Partition and Route.} During the indexing phase, each object $o$ is partitioned to the cluster with the highest probability according to $Prob_o$. 
%Once the partitioning is complete, the objects corresponding to a cluster are stored in a corresponding list. 
Once the partitioning is completed, the objects assigned to a cluster are stored in a corresponding list, which acts as an inverted file for these objects. Each object in this list is represented by a $d$-dimensional vector $o.emb$, and a geo-location $o.loc$, which will be utilized to calculate the relevance score for incoming queries. During the query phase, a given query $q$ is directed to the cluster that has the highest probability. Subsequently, the relevance scores between $q$ and all objects within the cluster are calculated and the top-k objects are selected as result objects.
% We partition each object $o$ to the cluster with the highest probability according to $Prob_o$ during the indexing phase. Once the partition is over, objects corresponding to a cluster are stored in the associated list. The objects in that list is presented by a $d$-dimensional vector $o.emb$ and a geo-location $o.loc$, which is used to compute relevance score with incoming queries. During the query phase, each query $q$ is routed to the cluster with the highest probability according to $Prob_q$. Then $q$ computes relevance score with all objects within the list of that cluster based on the relevance model.

An alternative way is routing queries (objects) to $cr$ clusters with the highest probabilities based on $Prob_q$ ($Prob_o$). Although this might boost query effectiveness by considering more objects in different clusters, it sacrifices efficiency as more objects need to be calculated for a query, leading to an accuracy-efficiency trade-off. 
%We demonstrate this trade-off in the experiment and users can adaptively set $nc$ based on their varying needs (shown in Section~\ref{sec:exp-efficiency}). 
%Our experiments showed that routing to a single cluster is sufficiently effective, hence we empirically assign each query or object to only one cluster.

% {\color{red} 
\noindent\textbf{Insertion and Deletion Policy.} When a new object comes, we convert it into an embedding using the trained relevance model and then assign it to specific clusters using the trained index. 
%As discussed in Section~\ref{sec:related}, in cases of frequent insertions, we periodically retrain the index. 
When an object is deleted, we simply remove it from the corresponding cluster. \revision{The time cost of the insertion operation is equivalent to the inference time of the neural networks, while the time cost of the deletion operation involves scanning the cluster lists and then deleting the object's id. The time costs of both operations are negligible.}
% }

\revision{Note that most existing ANNS indexes are static~\cite{luoSurveyDeepHashing2023,DBLP:journals/pami/WangZSSS18,DBLP:journals/pvldb/WangXY021}. When inserted data significantly differs in distribution from the existing data or when insertions occur frequently, periodically rebuilding the index is necessary to maintain high accuracy. This is because most ANNS indexes are based on the principle of organizing similar objects together, thereby routing queries to similar blocks to reduce search space. The functions determining which cluster each object belongs to are typically static, such as the distance between objects and the centroids of each cluster in an IVF index. When the distribution of embeddings changes significantly, these static functions can no longer accurately capture the new distribution, leading to a drop in performance. In our approach, we address this issue by only retraining the index, but not the relevance model.} 

% We demonstrate the robustness of our index when handling new POIs in our experiments. Notably, this insert policy requires the new insertions to be under stationary data distributions with existing objects, such as the new POIs being from the same city as the existing trained POIs. If the distribution of the inserted data significantly differs from the existing data, periodic retraining would be necessary to maintain accuracy, which is a common requirement for almost all vector databases.}

%Gao: the following does not help. better not mention 

%\noindent\textbf{Choice of $c$.} The choice of $c$ is important. Empirically, we recommend setting $c$ to approximately $\frac{n}{10,000}$. This is because ranking 10,000 objects by the relevance model is computationally feasible and does not notably compromise effectiveness. 


% If the clusters generated by our index are uniformly distributed, a larger $c$ would mean fewer objects and queries within each cluster. Consequently, the relevance model would have fewer objects to rank, thereby improving efficiency. However, a very high value of $c$ can lead to positive query-object pairs being assigned to different clusters, which could compromise the accuracy of our index. Hence, $c$ acts as a hyperparameter to control the trade-off between accuracy and efficiency. 

%\noindent\textbf{Cluster Evaluation and Reassignment.} 
\noindent\textbf{Cluster Evaluation.} After the training phase, we employ the trained index to produce clusters $C=\{C_1,C_2,\\ \cdots,C_{c}\}$, where $C_i$ represents cluster $i$. We use validation queries to evaluate the quality of the clusters. The validation queries are fed into the trained index and routed to a cluster. $C_{i}^{q}$ denotes a list containing the validation queries routed to $C_i$, $C_{i}^{o}$ denotes a list containing objects partitioned to $C_i$, and $||$ indicates the size of a list. We proceed to introduce two metrics to evaluate the quality of the clusters.


The first metric evaluates the precision of $C_i$, denoted as $P(C_i)$, representing the degree to which queries are aligned with their corresponding positive (relevant) objects in the same cluster, which is defined below: 
% \vspace*{-1em}
\begin{equation}
P(C_{i}) = \frac{1}{|C_{i}^{q}|} \sum\limits_{q_j \in C_{i}^{q}}\frac{|\text{pos}_{q_j}\cap C_{i}^{o}|}{|\text{pos}_{q_j}|}.
\label{eq:precision_cluster}
\end{equation}
Building upon this, we compute the average precision across all clusters, denoted as $P(C)$, which is defined as below: 
% \vspace{-0.5em}
\begin{equation}
P(C) = \frac{1}{\sum\limits_{C_{i} \in C}|C_{i}^{q}|} \sum_{C_i \in C} P(C_i) * |C_i^{q}|.
\label{eq:precision}
\end{equation}
%Clearly, a higher $P(C)$ indicates less effectiveness degradation caused by the index. 
Intuitively, a higher $P(C)$ indicates that the index is more effective.% degradation caused by the index. 

In addition, we also take into account efficiency concerns. For this purpose, we introduce another metric, the Imbalance Factor (IF)~\cite{johnson2019billion}, which measures the degree of balance across all clusters, denoted as $\text{IF}(C)$. The $IF(C)$ is formulated as: 
% \vspace{-0.5em}
\begin{equation}
\text{IF}(C) = \frac{\sum|C_{i}|^2}{(\sum|C_{i}|)^2},
\label{eq:IF}
\end{equation}
where $\text{IF}(C)$ is minimized when $|C_1|=|C_2|=\cdots=|C_{c}|$ according to the Cauchy-Schwarz Inequality. A higher imbalance factor indicates a more uneven distribution of clusters. When most objects are concentrated in a few large clusters, the imbalance factor increases significantly, which is undesirable for our task. Overall, our goal is to achieve high-quality clustering results characterized by higher $P(C)$ and lower $\text{IF}(C)$. In our index, with proper hyperparameters, our training process of the cluster classifier is able to obtain high-quality clusters. In the experiments, We study the quality of the clusters produced by our proposed index using these evaluation metrics %demonstrate this superiority 
(shown in Section~\ref{sec:exp-ablation}).


%\noindent\textbf{Cluster Reassignment.} 
% \subsubsection{Cluster Reassignment.}

%Inspired by the cluster reassignment and centroid refinement process used in the traditional cluster algorithms, we introduce a non-trivial cluster reassignment approach to further improve $P(C)$. 

%Once the learning process is completed, the index will produce $c$ clusters in the indexing phase. However, the precision of these clusters can vary significantly. Such variation indicates that queries routed to lower-precision clusters might be less effective compared to those routed to high-precision clusters. To enhance the queries' effectiveness, we propose to reassign objects in %certain 
%clusters, which further improves $P(C)$. The reassignment 
%decision 
%is based on two factors: $P(C_i)$ and a set precision threshold $\lambda$. If a cluster's precision is below $\lambda$, every object within that cluster will be reassigned to other clusters. We examine its $c$-cluster probability distribution and reassign it to a cluster that has the highest probability among all the clusters with precision surpassing the threshold $\lambda$. 

% %that not only has a precision surpassing the threshold $\lambda$ but also displays the highest probability when compared to other clusters meeting the same precision criteria.

%In the query phase, given that objects from low-precision clusters have been reassigned, we simply adjust the original routing procedure by bypassing the empty clusters, which introduces no additional time cost.

%\noindent\textbf{Complexity Analysis.} 




% \vspace*{-0.5em}


\subsection{Procedures and Analyses of \Framework}
\label{sec:workflow}
\begin{algorithm}[t]
    % \small
    \caption{Procedures of LIST.}
	\label{alg:workflow}
	\KwIn{A geo-textual object dataset $D$, a relevance model $R$, a index $I$, training \tkskqs set $Q_{\text{train}}$, and incoming \tkskqs set $Q$}
	\KwOut{The response $Res_{q}$ for each query $q \in Q$}
    \vspace*{1ex}
	// \textbf{Training Phase: } $Train(Q_{\text{train}}, D, R, I)$\\
    Train $R$ by $Q_{\text{train}}$, $D$ based on Eqaution~\ref{eq:loss}\;
    Employ $R$ to generate pseudo-labels based on Equation~\ref{eq:negative_pool}\;
    Employ pseudo-labels to train $I$ based on Equation~\ref{eq:MCL}\;
    \vspace*{1ex}
	// \textbf{Indexing Phase: } $Indexing(D)$\\
    \For{$o \in D$}{
        Transform $o.doc$ to $o.emb$ based on Equation~\ref{eq:DE}\;
        Transform $o.emb$, $o.loc$ to $x_o$ based on Equation~\ref{eq:representation}\;     
        Generate $Prob_{o}$ by $MLP$ based on Equation~\ref{eq:L2PO}\;
        Parition $o$ to cluster $C_i$ based on $Prob_{o}$\;
    }
    % {\bf return} ${C=\{C_i\}}$\;
    \vspace*{1ex}
    // \textbf{Query Phase: } $Search(q, C, R, I)$\\
    \For{$q \in Q$}{
        Transform $q.doc$ to $q.emb$ based on Equation~\ref{eq:DE}\;
        Transform $q.emb$, $q.loc$ to $x_q$ based on Equation~\ref{eq:representation}\;     
        Generate $Prob_{q}$ by $I$ based on Equation~\ref{eq:L2PO}\;        
        Route $q$ to cluster $C_i$ based on $Prob_{q}$\;
        $Res_{q} \leftarrow  \text{argTop-k}_{o \in C_i}  ST(q,o) $\;
        {\bf return} $Res_{q}$\;
    }    
\end{algorithm}
\noindent\textbf{Procedures of \Framework.}
The detailed procedures of \Framework are summarized at Algorithm~\ref{alg:workflow}. In the training phase, we train the proposed relevance model and index (lines 2-4). After that, in the indexing phase, we assign all objects to their corresponding clusters as inverted files (lines 6-10). In the query phase, given a new query $q$, we extract its features and then route it to a cluster $C_i$ by the index (lines 13-16). Consequently, we calculate the relevance score between $q$ and each object $o$ in that cluster by the relevance model, and the top-$k$ objects with the highest scores are returned to answer query $q$ (lines 17-18). \revision{In practice, the number of objects assigned to each cluster is  relatively small, and thus we evaluate all objects within the routed clusters
%which is a common exercise 
as it is in existing ANNS indexes.}

%\noindent\textbf{Training Phase.} First, we train our relevance model based on training queries (line 5), which is detailed in Section~\ref{sec:model}. Subsequently, based on the trained relevance model, we produce pseudo-negative labels and train our index (lines 6-7), as outlined in Section~\ref{sec:index}. 


% First, we train our relevance model as described in Section~\ref{sec:model}. Subsequently, based on the trained relevance model, we produce pseudo-negative labels and train our index as outlined in Section~\ref{sec:index}.



%\noindent\textbf{Indexing Phase.} In the indexing phase, objects are assigned to distinct clusters by our index. Specifically, each object $o$ is first transformed by the dual-encoder module (lines 11-12). After that, the cluster classifier produces the cluster distribution $Prob_{o}$ and partition objects according to $Prob_{o}$ (lines 13-14).



% Specifically, for each object $o$, its textual embedding $o.emb$ is obtained by the dual-encoder module, and then its feature can be extracted as Eq.~\ref{eq:representation}. After that, the cluster classifier outputs the corresponding cluster distribution, based on which we can get the cluster for the object. Here, the clusters of objects act as the inverted file for these spatial-textual objects, which helps to reduce the search space during the query phase.  


%\noindent\textbf{Query Phase.} In the query phase, given a new query $q$, the dual-encoder module is first employed to convert $q.doc$ into $q.emb$ (line 18). Then we route the query $q$ to a cluster $C_i$ by the \Index index (lines 19-21). Consequently, we calculate the relevance score between $q$ and each object $o$ in that cluster by the trained relevance model, which can be accelerated by the GPU (line 22). Then the top-$k$ objects with the highest scores are returned to answer query $q$ (line 23).


\noindent\textbf{Complexity Analysis.} Now we analyze the time and space complexity of \Framework. Assuming the dimensionality of the embedding is $d$, the total number of objects is $n$, \revision{the number of clusters is $c$}, and the number of layers in the MLP of the index is $l$. The embeddings $o.emb$ of objects are generated in advance. 

% When compared with other relevance models like DrW~\cite{liu2023effectiveness}, which has a time complexity of $O(nl^q(l^od+k')+l^q(2d^2+d))$ and space complexity of $O(n(l^od+2))$, with hyperparameters $l^q$, $l^o$ and $k'$ typically being tens, our relevance model exhibits superior efficiency in terms of both time and space complexities. 

For a given query, the time complexity of \Framework is $O((l-2)d^2+dc+\frac{n}{c}(d+2)+d)$. $O((l-2)d^2+dc)$ is the time complexity for our index (lines 15), which is the inference computation cost of Equation~\ref{eq:L2PO}. $O(\frac{n}{c}(d+2)+d)$ is the time cost of our relevance model (line 17). $\frac{n}{c}$ denotes the number of objects to be checked by the relevance model, which is approximately $\frac{1}{c}$ of the entire dataset. This is because of the even cluster distribution (Verified in Section~\ref{sec:exp-ablation}), which means approximately $\frac{1}{c}$ of the dataset needs to be visited. %Specifically, $O(\frac{nd}{c})$ is the computational cost of Equation~\ref{eq:textual-relevance}. $O(\frac{2n}{c})$ is the computational cost of Equation~\ref{eq:DSR_inference}, and $O(d)$ is the computational cost of Equation~\ref{eq:model_weight}. 
The space complexity of \Framework is $O((l-1)d+dc)+n(d+2)$. $O((l-1)d+dc)$ is the size of the MLP used by our index. $O(nd)$ represents the space required for storing pre-computed $o.emb$, and $O(2n)$ denotes the storage cost for geo-locations.

% \revision{When compared with other retrieve-and-rerank methods, such as using \tkskqs to retrieve $m$ objects and then employing DrW to rerank the retrieved objects (denoted as \tkskqs+DrW), \Framework still exhibits superior efficiency. }







==> intro.tex <==
% \vspace*{-0.2cm}
\section{Introduction}
\label{sec:intro}
With the proliferation of mobile Internet, spatio-textual (a.k.a geo-textual) data is being increasingly generated. Examples of spatio-textual data include (1) web pages with geographical information; (2) user-generated text content with location information, such as geo-tagged tweets and reviews related to local stores; (3) Points of Interest (POI) in local business websites or location-based apps~\cite{DBLP:journals/pvldb/ChenLCLBLGZ21}; (4) multimedia data that  contains both text and geographical location, like photos shared on social platforms that provide both textual descriptions and geographic location. Meanwhile, with the prevalence of smartphones, accessing and querying spatio-textual data has become increasingly frequent. This trend calls for techniques to process spatial keyword queries efficiently and effectively, which take query keywords and location as input and return objects that match the given requirements. \revision{An example query is to search for a `delicious pizza restaurant' that is close to the user’s location. A returned object could be a nearby restaurant named `Pizza Palace'.}

Spatial keyword queries have applications in many real-world scenarios such as geographic search engines~\cite{DBLP:conf/sigmod/ChenSM06}, location-based services~\cite{DBLP:conf/cikm/ZhouXWGM05}, and local web advertising tailored to specific regions~\cite{dong2021continuous}. To meet diverse user needs, various types of spatial keyword queries have been introduced~\cite{congEfficientRetrievalTopk2009,DBLP:conf/sigmod/ChenSM06,cary2010efficient,DBLP:journals/vldb/ChenCCJ21}. Among them, the \underline{T}op-\underline{k} KNN Spatial Keyword \underline{Q}uery (\tkskq)~\cite{congEfficientRetrievalTopk2009} retrieves the top-k geo-textual objects according to a ranking function that considers both textual and spatial relevance. Specifically, \tkskq computes textual relevance by traditional information retrieval models such as BM25 and TF-IDF~\cite{DBLP:journals/ftir/RobertsonZ09,DBLP:journals/tois/WuLWK08} and uses a linear function of distance between query location and object location to evaluate spatial relevance (as to be formulated in Section~\ref{sec:preliminary}). According to the experimental evaluation~\cite{liu2023effectiveness}, \tkskqs return more relevant objects compared to several other spatial keyword queries like the Boolean KNN Query~\cite{cary2010efficient}. Most of the existing studies~\cite{congEfficientRetrievalTopk2009,DBLP:conf/icde/FelipeHR08,DBLP:journals/tkde/LiLZLLW11, DBLP:conf/ssd/RochaGJN11} on spatial keyword queries focus on improving the efficiency of handling spatial keyword queries. 
As such, various indexes~\cite{DBLP:journals/vldb/ChenCCJ21} and corresponding query processing algorithms have been developed. 

\noindent\textbf{Motivations.} Despite various indexes~\cite{DBLP:journals/vldb/ChenCCJ21} have been developed to expedite the top-k search process of \tkskqs, the effectiveness of \tkskqs is limited. As discussed earlier, \tkskq uses traditional models such as BM25 to compute textual relevance, but these models rely on exact word matching to evaluate textual relevance and thus suffer from the word mismatch issue~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20,renRocketQAv2JointTraining2021,DBLP:conf/naacl/QuDLLRZDWW21}, e.g., synonyms that consist of different tokens may convey the same or similar meanings, which limits their effectiveness (as to be detailed in Section~\ref{sec:motivations}). \revision{For example, consider searching for an `Italian restaurant' on a location-based app like Foursquare. Even if a nearby restaurant named `Pasta House' exists, traditional models 
%may struggle to 
will not be able to retrieve this result because they cannot semantically match `Italian restaurant' with `Pasta House', it will receive %very low or even 
zero textual relevance score.}

%\revision{An example provided by~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20} illustrates this issue: the query `the bad guy in Lord of the Rings?' corresponds to the character `the villain Sauron'. Traditional models struggle to retrieve the result %this context 
% because they cannot semantically match `bad guy' with `villain'.} 

%For example, when a user searches for `nearby bar', nearby bars named `pub' or `tavern' will be ignored by these traditional models. 




% Another limitation arises from using the linear function of distance to calculate spatial relevance. This practice is based on an assumption that the user's spatial preference for geo-textual objects is a linear function of distance. However, this assumption was not examined previously and does not hold on our real-life datasets, where the spatial preference for geo-textual objects exhibits a significant (non-linear) decrease with the increase of distance. This mismatch with real-world situations results in limited effectiveness (as to be detailed in Section~\ref{sec:motivations}).


To improve the effectiveness of \tkskq, several deep learning based relevance models~\cite{liu2023effectiveness,DBLP:conf/sigir/DingCXHLZX23,DBLP:conf/aaai/ZhaoPWCYZMCYQ19} have recently been proposed, but they suffer from severe efficiency issue. \revision{For instance, DrW~\cite{liu2023effectiveness} employs the BERT model~\cite{devlin2018bert} to generate word embeddings and identifies top-k relevant terms from object description for each query keyword based on the word embeddings. It then uses an attention mechanism to aggregate the relevance scores between each keyword and its top-k relevant terms, determining the overall textual relevance. In our experiment, DrW takes over 7 seconds to answer a query in the Geo-Glue dataset using brute-force search. Moreover, to the best of our knowledge, there are no efficient indexes %specifically 
designed to expedite the top-k search process for these deep relevance models. %It uses the linear function of distance to calculate spatial relevance and 
} 



%To the best of our knowledge, there are no efficient indexes specifically designed to expedite the top-k search process for these deep relevance models. For example, the recently proposed DrW~\cite{liu2023effectiveness} employs the BERT model~\cite{devlin2018bert} to generate word embeddings, identifies top-k relevant terms from object description for each query keyword based on the word embeddings, and utilizes an attention mechanism to aggregate the relevance scores of every query keyword as the textual relevance. It also uses the linear function of distance as the spatial relevance. The interactions between word embeddings bring very high query latency. And it relies on interactions between the word embeddings of queries and objects, which cannot be pre-computed until the query-object pairs are given, therefore there is no efficient index designed for it (detailed in Section~\ref{sec:motivations}). 




% they have very high query latency for computing the relevance score due to their reliance on {\color{red}word} embeddings and complex neural networks (detailed in Section~\ref{sec:motivations}).
%to compute textual relevance based on word embeddings} 
% Although these approaches could achieve better effectiveness,   
% {\color{blue} word embeddings, i.e., high-dimensional dense vectors with semantic meaning.} 


%{\color{red}Lastly, %for spatial relevance, both \tkskq~\cite{congEfficientRetrievalTopk2009,DBLP:conf/icde/FelipeHR08,DBLP:journals/tkde/LiLZLLW11, DBLP:conf/ssd/RochaGJN11} and the state-of-the-art deep relevance model~\cite{liu2023effectiveness} %for \tkskqs~use %compute spatial relevance by a linear function of the distance between query location and object location to compute spatial relevance, but this practice does not fit real-world scenarios and leads to limited effectiveness.} 

%The implicit assumption behind this practice is that the user's geographical preference for geo-textual objects is a linear function of distance. However, this assumption was not examined previously and we find it does not hold on our real-life datasets. From our dataset, we find that the spatial preference for geo-textual objects %is not a linear function of distance, but exhibits a significant (non-linear) decrease with the increase of distance (detailed in Section~\ref{sec:motivations}). %This motivates us to design a more effective spatial relevance module.
%This motivates us to design a new spatial relevance module to better fit the real-world scenario. 
%An intuitive solution would be to employ an exponential function. However, our experiments indicate that this method is even less effective compared to the linear function (shown in Section~\ref{sec:exp-ablation}). 

% Although there exists deep relevance model~\cite{DBLP:conf/aaai/ZhaoPWCYZMCYQ19} designed for query-POI matching, which is essentially spatial keyword query, they cannot even outperform the \tkskq according to the experiment evaluation~\cite{liu2023effectiveness}. Recently, DrW~\cite{liu2023effectiveness} is proposed and is proven to outperform \tkskq.

%\noindent\revision{\textbf{Objective and Challenges.} In this paper, we aim to develop a new solution that effectively and efficiently answers spatial keyword queries. An intuitive approach is to design an index for existing deep learning models, such as DrW. However, these models suffer from high latency and are difficult to index. The obstacle arises from the complex word interaction functions, which rely on word embeddings to calculate the word-level similarity between query keywords and object descriptions for evaluating textual relevance. According to~\cite{guo2020deep}, these functions not only result in high latency but also cannot be pre-calculated until the input query-object text pairs are seen, making it challenging to build an index for them.}

\noindent\revision{\textbf{Objective and Challenges.} To this end, we aim to develop an efficient index for deep learning models to answer spatial keyword queries. However, these models, such as DrW, often suffer from high latency and it is difficult to design indexes for them due to their complex word interaction functions, which rely on word embeddings to calculate the word-level similarity between query keywords and object descriptions for evaluating textual relevance. According to~\cite{guo2020deep}, these functions not only result in high latency but also cannot be pre-calculated until the query-object text pairs are seen, making it challenging to build an index for them.}

\revision{To address this, we consider the embedding based spatial keyword queries, which capture the semantic meanings of query keywords and object descriptions into two separate embeddings and evaluate textual relevance based on the two embeddings. 
%
Many %language 
text %relevance 
models can be used for the embedding based spatial keyword queries, ranging from earlier Word2Vec~\cite{mikolov2013efficient} %embedding 
to the recent advancements in pre-trained language models~\cite{zhao2024dense}.
%, which offer effective techniques for generating embeddings.
} 
%Next, we elaborate on (1) how to develop a lightweight yet effective relevance model for embedding based spatial keyword queries and (2) how to design an index for embedding based spatial keyword queries.


% \revision{For the first objective, we propose a new relevance model that comprises three modules: a textual dual-encoder module, a novel learning based spatial relevance module, and a new weight learning module. The dual-encoder module %employs the BERT model to 
% converts query keywords %(e.g., `Italian restaurant') 
% and object descriptions %(e.g., store's title like `Pasta House') 
% into two separate embeddings and evaluates textual relevance %by calculating 
% the inner product %
% based on %between 
% the two embeddings. The learning-based spatial relevance module is designed to better fit real-world scenarios, thereby more effectively capturing spatial relevance. Existing relevance models, such as DrW and \tkskq, typically use the linear function of distance to calculate spatial relevance, assuming a linear relationship between user's spatial  preference and distance. However, this assumption was not examined previously and does not hold on our real-life datasets, thereby leading to limited effectiveness (as to be detailed in Section~\ref{sec:motivations}). To address this, the new spatial relevance module learns from real-world datasets to better evaluate spatial relevance. Finally, a weight learning module is proposed to adaptively learn a weight to balance the textual and spatial relevance.}

% \noindent\textbf{Objectives.} 
% To address the aforementioned issues,
% %and develop an effective and efficient solution to answering the \tkskq query, 
% this work aims to (1) design an embedding based lightweight yet effective spatio-textual relevance model as the ranking function, and (2) design a novel index to speed up high-dimensional embedding based spatial keyword queries.
% To address the aforementioned issues, this work aims to (1) design a lightweight yet effective relevance model, %{\color{red}for embedding spatial keyword queries}, 
% and (2) design an index to expedite the top-k search process of the proposed relevance model.
%{\color{red} embedding spatial keyword queries.}%the proposed deep learning based relevance model.

% For the first objective, we propose a lightweight yet effective relevance model for embedding based spatial keyword queries, which capture the semantic meaning of query keywords in one high-dimensional embedding. The relevance model comprises three modules: a textual dual-encoder module, a novel learning based spatial relevance module, and a new weight learning module. The dual-encoder module converts query keywords and object descriptions \revision{(e.g., query keywords like `delicious Chinese restaurant' and object descriptions like a restaurant's title named `Sichuan restaurant')} into two separate embeddings and evaluates textual relevance based on the two embeddings. To overcome the limitation of linear distance function, as explained earlier,  we propose a new learning-based spatial relevance module, which is capable of learning from real-world datasets to better evaluate spatial relevance. Additionally, a weight learning module is proposed to adaptively learn a weight to balance the textual and spatial relevance.

%For the second objective, 

\revision{The challenge lies in developing an index for embedding based spatial keyword queries.}
%
Existing geo-textual indexes are developed based on traditional models such as BM25 and TF-IDF, which %rely on exact word matching to prune low textual relevance. These geo-textual indexes 
cannot be used to handle embedding based spatial keyword queries. Although Approximate Nearest Neighbor Search (ANNS) indexes~\cite{qin2020similarity,DBLP:journals/pami/WangZSSS18,DBLP:journals/pvldb/WangXY021} are designed for embedding retrieval, these ANNS indexes do not consider %take into account 
the spatial factor, which is essential for spatial keyword queries. Directly using these ANNS indexes for embedding based spatial keyword queries results in severe degradation of effectiveness (as to be shown in Section~\ref{sec:exp-effectiveness}). An intuitive idea is to adapt these ANNS indexes to incorporate the spatial factor. For instance, the IVF index~\cite{jegouProductQuantizationNearest2011} clusters embeddings using the K-means algorithm and route queries to a small number of close clusters to reduce the search space. However, incorporating spatial factors into the K-means algorithm is challenging as it is hard to set the weight to balance spatial and embedding similarities during index construction. Manually setting the weights is not only laborious but also ineffective, resulting in inferior effectiveness (as to be shown in Section~\ref{sec:exp-effectiveness}). It is still an open problem to design an effective and efficient ANNS index to support embedding based spatial keyword queries.

To fill this gap, we develop a new machine learning based ANNS index \revision{that is applicable to any relevance models for embedding based spatial keyword queries only if query and objects are represented by two embeddings.} To %avoid manually balancing spatial and textual factors
cluster both spatial and textual relevant objects together without manually setting the weight between spatial relevance and textual relevance, our proposed index utilizes the learning-to-cluster technique, which was originally developed for image clustering, to learn from pairwise relevant and irrelevant query-object pairs, thereby clustering relevant objects and queries together while separating the irrelevant ones. Existing learning-to-cluster studies~\cite{Hsu16_KCL,Hsu18_L2C} demonstrate that high-quality pairwise similar/dis-similar labels are essential for training. Although these pairwise labels are easy to obtain for images,
such pairwise positive labels between %spatial keyword 
queries and %geo-textual 
objects in our problem are very sparse%(click-through or human annotation, detailed in Section~\ref{sec:exp-setup})
, and high-quality negative labels are absent. Additionally, when the number of clusters is large, the existing learning-to-cluster technique will produce a highly skewed cluster distribution~\cite{Hsu16_KCL}, which will hurt the index's efficiency if the index is built based on the cluster results. To address these challenges, we propose a novel pseudo-negative label generation method, which employs the trained relevance model to produce high-quality pseudo-negative labels. %{\color{red}Through these informative labels,}
%{\color{red} Through these informative negative labels combined with ground-truth positive (relevant) labels (e.g., click-through or human annotation, detailed in Section~\ref{sec:exp-setup}),} %enable 
Through these informative labels, our index learns to precisely cluster relevant queries and objects together while separating the irrelevant ones, thereby producing a precise and balanced clustering result and constructing an effective and efficient ANNS index.

\revision{We call the proposed index as \Framework, which \underline{l}earns to \underline{i}ndex \underline{s}patio-\underline{t}extual data for answering embedding based spatial keyword queries. \Framework employs a relevance model to pre-compute embeddings for geo-textual objects, and learns to index these embeddings. %uses the proposed index to cluster the relevant objects together while separating irrelevant ones. 
Given an embedding-based spatial keyword query, \Framework routes the query to a subset of clusters to reduce the search space. Subsequently, the relevance model is applied to re-rank the retrieved objects within the relevant clusters (as to be detailed in Section~\ref{sec:LIST}).}

\revision{In addition, we improve the spatial relevance for embedding based spatial keyword queries. Existing relevance models such as DrW typically %compute spatial relevance using
use the linear function of distance, %between query and object locations, 
assuming that spatial preference decreases linearly with distance. %The implicit assumption behind this practice is that the spatial preference for geo-textual objects is a linear function of distance. 
However, this assumption was not examined previously. We find it does not hold on our real-life datasets, and that  the spatial preference %for geo-textual objects 
exhibits a significant (non-linear) decrease with the increase of distance (as to be detailed in Section~\ref{sec:motivations}). This motivates us to design a new spatial relevance model to fit this real-world pattern better. A straightforward approach would be to employ an exponential function of distance. However, our experiments indicate that this simple method is even less effective compared to the linear function (as to be shown in Section~\ref{sec:exp-ablation}).} 
%
\revision{Instead, we design a learning based spatial relevance model, which learns from real-world datasets to better evaluate spatial relevance. The spatial model is built on two real-world patterns: (1) spatial relevance increases as distance decreases, and (2) spatial relevance increases in a stepwise manner rather than continuously as distance decreases. Therefore, we designed the model as a learnable monotonic step function. Additionally, we introduce a weight learning module to adaptively learn a weight for embedding based spatial keyword queries to balance the textual and spatial relevance. 
%These two components can integrate with various language processing techniques that can transform query keywords and object descriptions into separate embeddings to form a lightweight yet effective relevance model for embedding based spatial keyword queries.
%which is designed to be a monotic step function.
}


%Based on the two techniques proposed above, namely the lightweight yet effective relevance model and the machine learning based ANNS index, we propose a new solution, which \underline{l}earns to \underline{i}ndex \underline{s}patio-\underline{t}extual data for answering embedding based spatial keyword queries (called \Framework). \Framework employs the  relevance model to pre-compute embeddings for geo-textual objects and uses the proposed index to cluster the relevant objects together while separating irrelevant ones. Given embedding based spatial keyword queries, \Framework routes queries to a subset of clusters to reduce the search space. Subsequently, the relevance model is applied to re-rank the retrieved objects within the relevant clusters (detailed in Section~\ref{sec:LIST}).

% {\color{red}
% In this study, to %address 
% achieve the two %open problems,
% objectives,
% %to answer \tkskqs effectively and efficiently,  
% we propose a novel solution, which \underline{l}earns to \underline{i}ndex \underline{s}patio-\underline{t}extual data for answering embedding based spatial keyword queries. %Here, embedding based spatial keyword queries represent the semantic meaning of query keywords with a single high-dimensional embedding. 
% We denote this retriever by \Framework, which is featured with two new components. First, \Framework~proposes a lightweight
% and effective relevance model, which comprises three modules: a textual dual-encoder module that transforms query keywords and object descriptions into an embedding separately and evaluate textual relevance based on these embeddings,  %to capture textual relevance and transform spatial keyword queries and geo-textual objects into their embedding-based forms, 
% a novel learning based spatial relevance module that learns to estimate spatial relevance, 
% and a new weight learning module}. 

% Second, \Framework develops a novel machine learning based ANNS index. {\color{red} For embedding based spatial keyword queries and geo-textual objects, our proposed index utilizes the learning-to-cluster technique, which was developed for image clustering, to cluster relevant objects and queries together while separating the irrelevant ones. This approach enables our proposed index to avoid manually balancing the importance between the textual and spatial factors.}
% % our proposed index utilizes the learning-to-cluster technique, which was developed for image clustering in the field of computer vision,
% %which was developed for computer vision applications, 
% % to cluster relevant geo-textual objects and queries together {\color{red} while separating the irrelevant ones for index construction}. {\color{red}This approach enables our proposed index to avoid manually balancing the importance between the textual and spatial factors and utilize neural networks to learn to cluster geo-textual objects and route {\color{red} embedding based} spatial keyword queries to relevant clusters.}
% %For the queries, we route them by neural networks to a subset of clusters to reduce the search space, where objects within the cluster will be reranked by a relevance model. 
% Existing learning-to-cluster techniques~~\cite{Hsu16_KCL,Hsu18_L2C} 
% %employ neural networks to cluster image data in an end-to-end way and 
% rely on partial pairwise similar/dis-similar relationships of images for training. {\color{red}Although these pairwise labels are easy to obtain for images,
% %obtained from existing image labels. 
% %However, 
% such pairwise positive labels for spatial keyword queries and geo-textual objects in our problem are very sparse, and high-quality negative labels are absent.} %which are important for learning-to-cluster. 
% %Training with low-quality negative labels will result in indistinguishable cluster results. 
% Additionally, when the number of clusters exceeds the number of image classes, the existing learning-to-cluster technique will produce a highly skewed cluster distribution~\cite{Hsu16_KCL}, which will hurt the {\color{red}index's efficiency}. To address these challenges, we propose a novel pseudo-negative label generation method, which employs the trained relevance model to produce high-quality pseudo-negative labels. {\color{red} By training with these informative negative labels %combined with 
% and ground-truth positive (relevant) labels (e.g., click-through or human annotation, detailed in Section~\ref{sec:exp-setup}), %enable 
% our index learns to precisely cluster relevant queries and objects together while separating the irrelevant ones, thereby producing a precise and balanced clustering result and construct an both effective and efficient ANNS index.}
%both spatial and textual information, thereby clustering relevant objects and queries together while separating irrelevant objects and queries.


% \item \textbf{New %Spatial 
% Relevance Model.} We develop a lightweight yet effective relevance model. It is featured with a dual-encoder module to convert query keywords and object descriptions into two separate embeddings and compute textual relevance based on the two embeddings, a novel learning-based spatial relevance module to learn from real-word datasets to better evaluate the spatial relevance, and a new weight learning mechanism to determine the weights between textual and spatial relevance. 

The contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*,topsep=0pt]
\item \textbf{New Index.} We develop a novel machine learning based ANNS index that is tailored for embedding based spatial keyword queries and accelerating the top-k search process of the proposed deep relevance model. Different from existing ANNS indexes, it utilizes the learning-to-cluster technique to cluster relevant objects and queries together while separating the irrelevant ones. To build an effective and efficient index, we propose a novel pseudo-label generation approach. To the best of our knowledge, this is the first index designed for embedding based spatial keyword queries and deep relevance model. Additionally, this is the first geo-textual index that employs neural networks for retrieval without relying on an explicit tree structure.% and corresponding heuristic query processing algorithms. 


\item \revision{\textbf{New Spatial Relevance Model.} We develop a novel learning based spatial relevance module, which is capable of learning from real-world datasets to better evaluate the spatial relevance. This model can integrate with various 
%%language processing techniques 
textual relevance models 
%to develop a relevance model 
for embedding based spatial keyword queries.}

% \item \textbf{Extensive Experiments.} We extensively evaluate the effectiveness and efficiency of our proposed \Framework solution %and its two main components, i.e., relevance model and index, 
% on three real-world datasets. Experimental results show that %(1) 
% \Framework significantly outperforms the state-of-the-art baseline algorithms for effectiveness by an improvement up to 19.21\% and 12.79\% in terms of NDCG@1 and Recall@10 respectively and is three orders of magnitude faster than the most effective baseline. %; (2) Our proposed relevance model outperforms the state-of-the-art relevance models in terms of NDCG@1 and Recall@10 by a margin of 18.36\%, and 10.22\%, respectively. (3) Our proposed index outperforms the most effective baseline indexes in terms of effectiveness on the large-scale dataset with three orders of magnitude faster querying speed. 
% %Our implementation is released at \url{https://github.com/Heisenberg-Yin/LIST}.

\item \revision{\textbf{Extensive Experiments.} We extensively evaluate the effectiveness and efficiency of our solution \Framework
%and its two main components, i.e., relevance model and index,
on three real-world datasets. Experimental results show that (1) our lightweight embedding based relevance model
%\Framework 
significantly outperforms the state-of-the-art relevance models for effectiveness by an improvement up to 31.60\% and 59.92\% in terms of NDCG@1 and Recall@10, respectively; %and is three orders of magnitude faster than the most effective baseline; 
(2) \Framework outperforms existing state-of-the-art indexes on the three datasets, providing a better trade-off between effectiveness and efficiency.} 

%; (2) Our proposed relevance model outperforms the state-of-the-art relevance models in terms of NDCG@1 and Recall@10 by a margin of 18.36\%, and 10.22\%, respectively. (3) Our proposed index outperforms the most effective baseline indexes in terms of effectiveness on the large-scale dataset with three orders of magnitude faster querying speed. 
%Our implementation is released at \url{https://github.com/Heisenberg-Yin/LIST}.




\end{itemize}


==> problem-statment.tex <==
\section{Problem Statement and Motivations}
\label{sec:problem-statement-and-motivations}
\subsection{Preliminary}
\label{sec:preliminary}
We consider a geo-textual object dataset $D$, where each geo-textual object $o\in D$ has a location description $o.loc$ and a textual description $o.doc$. The location description $o.loc$ is a two-dimensional GPS coordinate composed of latitude and longitude. The textual description $o.doc$ is a document that describes the object. The Top-k KNN Spatial-Keyword Query (\tkskq)~\cite{congEfficientRetrievalTopk2009} is defined as follows.


\noindent\textbf{Top-k KNN Spatial-Keyword Query (TkQ):} Given a query $q=\langle loc, doc, k\rangle$, where $q.doc$ denotes the query keywords, $q.loc$ is the query location, and $q.k$ is the number of returned objects, we aim to retrieve $k$ objects with the highest relevance scores $ST(q,o)$:
\begin{equation}
\begin{aligned}
    ST(q,o) = (1-\alpha) \times SRel(q.loc, o.loc) + \\
    \alpha \times TRel(q.doc, o.doc).
\end{aligned}
\label{eq:TkSKQ_rank}
\end{equation}
A higher score $ST(q,o)$ indicates higher relevance between the given query $q$ and object $o$. In this context, $SRel(q.loc, o.loc)$ denotes the spatial relevance between $q.loc$ and $o.loc$ and is often calculated by $1-SDist(q.loc, o.loc)$ in previous studies~\cite{congEfficientRetrievalTopk2009,DBLP:conf/icde/FelipeHR08,DBLP:journals/tkde/LiLZLLW11, DBLP:conf/ssd/RochaGJN11,liu2023effectiveness}, where $SDist(q.loc, o.loc)$ represents the spatial closeness and is usually computed by the normalized Euclidean distance: $SDist(q.loc, o.loc)=\frac{dist(q.loc, o.loc)}{dist_{max}}$. Here, $dist(q.loc, o.loc)$ denotes the Euclidean distance between $q.loc$ and $o.loc$, and $dist_{max}$ is the maximum distance between any two objects in the object dataset. $TRel(q.doc, o.doc)$ denotes the text relevance between $p.doc$ and $q.doc$ and is computed by traditional information retrieval models like BM25~\cite{DBLP:journals/ftir/RobertsonZ09} in previous studies~\cite{congEfficientRetrievalTopk2009,DBLP:conf/icde/FelipeHR08,DBLP:journals/tkde/LiLZLLW11, DBLP:conf/ssd/RochaGJN11}, and then normalize to a scale similar to spatial relevance. $\alpha \in [0,1]$ is a weight parameter to balance the spatial and text relevance. 





\subsection{Data Analysis and Motivations}
\label{sec:motivations}

\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/term-match.pdf}
    \caption{Word Mismatch Analysis}
    \label{fig:term-match}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{fig/CDF.pdf}
    \caption{Spatial Relevance Analysis}
    \label{fig:cdf_distribution}
\end{subfigure}
\caption{Figure~\ref{fig:term-match} shows the percentage distribution of ground-truth positive query-object pairs based on the number of matching terms on the Beijing dataset. Figure~\ref{fig:cdf_distribution} compares the CDF of spatial distance for ground-truth positive query-object pairs and the linear distribution on the Beijing dataset.}
\label{fig:spatial_relevance_score}
\end{figure}



\noindent\textbf{Word Mismatch.} As discussed in Section~\ref{sec:intro}, \tkskq~\cite{congEfficientRetrievalTopk2009,DBLP:conf/icde/FelipeHR08,DBLP:conf/ssd/RochaGJN11} typically uses traditional information retrieval methods such as BM25 and TF-IDF~\cite{DBLP:journals/ftir/RobertsonZ09,DBLP:journals/tois/WuLWK08} to compute textual relevance. These models rely on exact word matching to compute textual relevance and thus suffer from the word mismatch issue, which reduces their effectiveness. We further illustrate this issue in the real-world dataset that contains query-object ground-truth pairs. The details on the data are given in Section~\ref{sec:exp}. As shown in Figure~\ref{fig:term-match}, in the Beijing dataset, nearly 20\% of the ground-truth query-object positive (relevant) pairs have no overlap of words. This indicates that objects relevant to the query may receive a low or even zero textual relevance from these models. For instance, given a search `nearby drugstore', if the search engine employs the BM25 to determine textual relevance, a drugstore labeled as `pharmacy' would get a textual relevance score of zero, although the two terms convey the same meaning.


\noindent\textbf{Efficiency.} To address the word mismatch issue, several recent studies~\cite{liu2023effectiveness,DBLP:conf/aaai/ZhaoPWCYZMCYQ19,DBLP:conf/sigir/YuanLLZYZX20} have utilized deep learning techniques to evaluate textual relevance, thereby enhancing ranking effectiveness. However, these methods rely on word embeddings and complex neural networks to compute textual relevance, resulting in high querying latency. For instance, DrW~\cite{liu2023effectiveness} identifies the top-k relevant words from each object's description for each query word based on their word embeddings, and then aggregates the scores of these word pairs using an attention mechanism to compute the textual relevance. On the Geo-Glue dataset, which comprises 2.8 million objects, DrW takes more than 7 seconds to answer a query on average in our experiment, which aligns with the results reported in~\cite{liu2023effectiveness}. This makes them unsuitable as a retriever for practical geo-textual object retrieval applications, although they can be used as re-rankers for a small number of objects returned by a retriever.


\noindent\textbf{Motivations of \Framework.} As discussed in the last paragraph, incorporating deep textual relevance into spatial keyword queries has presented significant efficiency challenges. However, as discussed in Section~\ref{sec:related}, the first category of deep text relevance model, namely word interaction based deep relevance models, such as DrW~\cite{liu2023effectiveness}, which rely on word interaction modules and word embeddings to compute textual relevance, are not efficient for online computation and retrieval by a specifically designed index. Therefore, \revision{we consider embeddings based spatial keyword queries, which capture the semantic meaning of query keywords and object descriptions into two separate embeddings. Then the challenge lies in how to develop an index for embedding based spatial keyword queries as discussed in Introduction.}%developing a new lightweight yet effective relevance model and a new index to accelerate the top-k search process for spatial keyword queries based on the proposed deep relevance model is in demand. %such  models due to its reliance on complex neural networks and word embeddings. 
%For the first objective, %we introduce embedding based spatial keyword queries and 
%we develop a lightweight yet effective deep relevance model for embedding based spatial keyword queries. 

%For the second objective, 
%Existing geo-textual indexes~\cite{DBLP:journals/vldb/ChenCCJ21} developed for spatial keyword queries are designed based on traditional retrieval models such as BM25 and cannot be used to handle embedding based spatial keyword queries. %dense retrieval models. Existing ANNS indexes, which are discussed in Section~\ref{sec:related}, do not consider spatial factors. Directly employing existing ANNS indexes for spatial keyword queries will result in severe degradation of effectiveness (shown in Section~\ref{sec:exp-effectiveness}). Simply adapting existing ANNS indexes, such as the IVF index, to incorporate spatial factors will cause even more severe effectiveness degradation, as it is hard to manually set a weight to balance spatial and textual similarities (as to be shown in Section~\ref{sec:exp-effectiveness}). It is still an open problem to design a new ANNS index to support embedding based spatial keyword queries.%accelerate the top-k search process of the deep learning based relevance model.



\noindent\textbf{Spatial Relevance.} 
\revision{Previous studies, such as TkQ~\cite{congEfficientRetrievalTopk2009} and DrW~\cite{liu2023effectiveness}, typically compute spatial relevance by $1-SDist(q.loc,o.loc)$.}
%\tkskq~\cite{congEfficientRetrievalTopk2009,liu2023effectiveness} typically computes spatial relevance by $1-SDist(q.loc,o.loc)$. 
The implicit assumption behind this linear function is that the user's geographical preference for geo-textual objects is a linear function of distance. However, this assumption was not examined previously and we found it does not hold on our real-life datasets. In Figure~\ref{fig:cdf_distribution}, we illustrate this issue by comparing the cumulative distribution function (CDF) of ground-truth positive (relevant) query-object pairs with the `Linear Distribution', a linearly ascending hypothetical scenario that positive query-object pairs are uniformly distributed across the range $[0,1]$. This figure shows a sharp increase in the CDF of ground-truth positive pairs for $SDist(q.loc,o.loc)$ below 0.1, a pattern that %does not align with any known distribution and 
greatly differs from the hypothetical scenario. This motivates us to design a new spatial relevance module to better fit the real-world scenario. An intuitive solution would be to employ an exponential function. However, our experiments indicate that this method is even less effective compared to the linear function (as to be shown in Section~\ref{sec:exp-ablation}).


% \subsection{Problem Statement}
% \label{sec:problem-statement}
\noindent\textbf{Problem Statement.}\revision{ We aim to develop an ANNS index for deep learning based relevance models designed for embedding based spatial keyword queries, where query keywords and object descriptions are represented as two separate embeddings. %The index is applicable to both previous spatial relevance and our proposed spatial relevance. 
}
%(1) design a lightweight yet effective relevance model, and (2) develop an index to expedite the top-k search process of the proposed relevance model.


==> related.tex <==
% \vspace{-0.5em}
\section{Related Work}
\label{sec:related}
% \vspace{-0.5em}

\noindent \textbf{Spatio-Textual Relevance Models.}
%\label{sec:geo-textual-rank}
Spatial keyword queries have attracted extensive attention and many types of spatial keyword queries~\cite{congEfficientRetrievalTopk2009,DBLP:conf/sigmod/ChenSM06,cary2010efficient} have been proposed. Among them, Top-k KNN Spatial Keyword Query (\tkskq)~\cite{congEfficientRetrievalTopk2009} aims to retrieve top-k geo-textual objects based on a ranking function that evaluates both spatial and textual relevance.
%and is shown to return more relevant objects than other types of spatial keyword queries in an experiment evaluation~\cite{liu2023effectiveness}. 
%Spatial relevance is usually computed by the distance between a query and an object. 
Specifically, \tkskq computes the textual relevance with traditional retrieval models like BM25 and TF-IDF~\cite{DBLP:journals/ftir/RobertsonZ09,DBLP:journals/tois/WuLWK08} and exploits a simple linear function of distance for spatial relevance. However, these traditional methods have limited effectiveness.%However, these retrieval traditional models face the word mismatch issue, limiting their effectiveness. 


To enhance the effectiveness, several deep learning based methods~\cite{DBLP:conf/aaai/ZhaoPWCYZMCYQ19,liu2023effectiveness,DBLP:conf/sigir/DingCXHLZX23}
%,DBLP:conf/sigir/YuanLLZYZX20,DBLP:conf/kdd/HuangWSFHYL21}  
have been developed for query-POI matching, which is essentially spatial keyword query. PALM~\cite{DBLP:conf/aaai/ZhaoPWCYZMCYQ19} considers geographic information by using location embedding techniques and combines it with textual word semantic representations for query-POI matching. 
%It utilizes stacked CNNs and self-attention layers to estimate relevance scores between queries and POIs. 
DrW~\cite{liu2023effectiveness} computes the deep textual relevance on the term level of query keywords and object descriptions. It uses the attention mechanism to aggregate the scores of each term for spatial keyword queries and design a learning-based method to learn a query-dependent weight to balance textual and spatial relevance. MGeo~\cite{DBLP:conf/sigir/DingCXHLZX23} employs a geographic encoder and a multi-modal interaction module, treating geographic context as a new modality and using text information as another modality. MGeo aligns these two modalities into the same latent space and computes relevance scores based on the produced representations. 
%
However, these deep learning based methods focus on improving the effectiveness but ignore the efficiency issue. 

Different from previous %spatio-textual 
deep learning based relevance models that rely on word embeddings and complex models to compute textual relevance, %our proposed model employs a dual encoder module to transform query keywords and object descriptions into two embeddings, computes textual relevance based on two embeddings, and we also propose a new learning-based spatial module to learn from real-world datasets to better estimate spatial relevance. 
\revision{%our proposed relevance model is developed for 
we consider embedding based spatial keyword queries, which transform query keywords and object descriptions into two separate embeddings and computes textual relevance based on the two embeddings. We also propose a new learning based spatial module to learn from real-world dataset to better estimate spatial relevance.}


\noindent \textbf{Spatio-Textual Indexes.} 
Various spatio-textual indexes~\cite{DBLP:conf/sigmod/ChenSM06,cary2010efficient,DBLP:conf/icde/FelipeHR08,congEfficientRetrievalTopk2009, DBLP:journals/tkde/LiLZLLW11, DBLP:conf/ssd/RochaGJN11, DBLP:conf/icde/ZhangZZL13,tao2013fast,vaid2005spatio,DBLP:conf/cikm/GobelHNB09,DBLP:conf/cikm/ZhouXWGM05,DBLP:conf/sigmod/LuLC11,DBLP:conf/edbt/ZhangTT13,DBLP:conf/icde/ZhangOT10,DBLP:conf/icde/ZhangCMTK09, DBLP:journals/pacmmod/Sheng0F00C023,DBLP:conf/gis/Liu022} have been designed to efficiently answer spatial keyword queries. However, they are all designed for traditional retrieval models (e.g., TF-IDF), and 
are unsuitable for accelerating the top-k search process of these deep learning based methods. %for embedding based retrieval models used by deep learning based methods. 

%We are aware that 
Several indexes~\cite{DBLP:journals/www/QianXZZZ18,DBLP:journals/geoinformatica/ChenXZZLFZ20} have been introduced to incorporate semantic representations into the \tkskq scheme. 
%NIQ-Tree~\cite{DBLP:journals/www/QianXZZZ18} employs a Quad-tree to index objects by their geo-locations. Within each leaf node, objects are further indexed by the iDistance index~\cite{jagadishIDistanceAdaptiveTree2005} and inverted file index based on their terms and vectors produced by the LDA model~\cite{DBLP:journals/jmlr/BleiNJ03}. 
For example, S$^2$R-Tree~\cite{DBLP:journals/geoinformatica/ChenXZZLFZ20} projects the word embeddings to
an $m$-dimensional vector using a pivot-based technique ($m$ as low as 2). Consequently, it employs R-trees to index objects based on their geo-locations and $m$-dimensional vectors hierarchically. When the dimensionality reaches hundreds, which are common for embeddings, such methods are no better than a linear scan %solution 
due to the curse of dimensionality~\cite{indyk1998approximate}. 

Additionally, there exists a learned geo-textual index called WISK~\cite{DBLP:journals/pacmmod/Sheng0F00C023}, 
%has been proposed recently, 
which utilizes query workloads to partition
%s objects based on their location and keyword frequency 
geo-textual data to build a tree-based index and employ reinforcement learning techniques to optimize the index. However, WISK is designed for spatial keyword range queries, which treats query keywords and query region as Boolean filters, only retrieves objects containing all the query keywords within the given query region, and is not designed to support other queries like the \tkskq, which uses keywords to compute textual relevance.

Different from previous spatio-textual indexes developed to expedite the top-k search for a ranking function that uses traditional relevance models %(which is called sparse retrieval), 
like BM25 and TF-IDF, which depend on exact word matching to compute textual relevance, our goal is to design an index that accelerates the top-k search for a deep learning based relevance model \revision{that is developed for embedding based spatial keyword queries.} %(which is called dense retrieval)
It is still an open problem for geo-textual data.

\noindent \textbf{Deep Textual Relevance Models and Approximate Nearest Neighbor Search Indexes.}
%
%The recent spatio-textual relevance models are highly related to the deep text relevance models, which 
Our work is related to deep textual relevance models and the corresponding Approximate Nearest Neighbor Search (ANNS) index techniques. 
%
The deep textual relevance models can be broadly classified into two categories: interaction-focused models and representation-focused models~\cite{guo2020deep}. The first category of models (e.g., ARC-II~\cite{DBLP:conf/nips/HuLLC14} and MatchPyramid~\cite{DBLP:conf/aaai/PangLGXWC16}) calculates the word-level similarity between queries and documents for textual relevance. DrW~\cite{liu2023effectiveness} belongs to this category. Although this category of methods may have better effectiveness, these methods are usually computationally expensive. The second category of models (e.g., DSSM~\cite{huang2013learning}) extracts global semantic representation for input text and uses functions like the inner product to compute the relevance score between representations. This category of models used to be less effective than the first category of models. However, with the emergence of %the dual-encoder architecture~\cite{DBLP:conf/emnlp/KarpukhinOMLWEC20,DBLP:conf/icml/GuuLTPC20}, which employs 
Pre-trained Large Language Models (PLMs), which extract global semantic representation from textual content, it has become a well-established paradigm in document retrieval~\cite{DBLP:journals/tois/GuoCFSZC22,DBLP:journals/corr/abs-2211-14876,ECML_23_zhou2023master_dense_retrieval,SIGIR_23_wen2023offline_dense_retrieval,DBLP:conf/naacl/QuDLLRZDWW21}. For the second category of methods, to support efficient online retrieval, the learned sentence embeddings are usually pre-computed offline and indexed by the ANNS indexes~\cite{guo2020deep}. Note that, models in the first category like DrW~\cite{liu2023effectiveness} are not efficient for online computation and retrieval %like the models in the second category 
since the complex word interaction function cannot be pre-calculated until we see the input query-object pairs according to~\cite{guo2020deep}.

%\subsection{Approximate Nearest Neighbor Search indexes}
%\label{sec:ann}
%\noindent \textbf{Approximate Nearest Neighbor Search Indexes.}
%Computing the inner product or Euclidean distance between the query vector and all objects' vectors exhaustively is impractical. 
ANNS indexes are developed to expedite the top-k search on high-dimensional embeddings.
%, which sacrifices some accuracy to achieve faster search speeds. 
These techniques can be broadly categorized into two types. The first type focuses on searching a subset of the database. The representative methods include inverted file index (IVF) based methods~\cite{DBLP:journals/pami/BabenkoL15,jegouProductQuantizationNearest2011,wang2020deltapq}, hashing-based methods~\cite{luoSurveyDeepHashing2023, liu2014sk, liu2019lsh,zheng2020pm}, and graph-based methods~\cite{malkovEfficientRobustApproximate2020, DBLP:journals/pvldb/WangXY021}. These ANNS indexes typically rely on heuristic algorithms to find a subset of candidates. Specifically, Inverted File Index (IVF)~\cite{jegouProductQuantizationNearest2011} partitions data into clusters using the k-means algorithm and routes queries to a subset of close clusters based on the query's distance to the clusters' centroids. Graph-based algorithms like Hierarchical Navigable Small World (HNSW) index~\cite{malkovEfficientRobustApproximate2020} construct proximity graphs and perform a beam search on the graph for a given query to find similar embeddings. Hashing-based methods like Locality-Sensitive Hashing (LSH) index~\cite{DBLP:journals/corr/WangSSJ14} generate top-k candidates by hashing vectors into buckets and then retrieving the closest items from those buckets as candidates. The other type aims to accelerate the search process itself, such as quantization-based methods~\cite{jegouProductQuantizationNearest2011, DBLP:journals/pami/GeHK014,gao2019beyond, guoAcceleratingLargeScaleInference2020,DBLP:journals/pami/GeHK014}. 


Our method belongs to the first category and is orthogonal to the second category. Our proposed index differs from previous ANNS indexes in 
two aspects: (1) Our proposed index is designed for embeddings based spatial keyword queries. In contrast, existing ANNS indexes are designed for embedding retrieval and do not work well when being adapted to embedding based spatial keyword queries (to be shown in Section~\ref{sec:exp-effectiveness}). %In contrast, existing ANNS indexes are only for textual relevance. 
%and do not work well when being adapted to the spatio-textual relevance model (to be shown in Section~\ref{sec:exp-effectiveness}).
(2) Existing ANNS techniques are based on heuristic methods. If we want to incorporate spatial factor into the existing ANNS techniques, it is unavoidable to balance the weight between spatial and embedding relevance, which is however challenging. To avoid this, our proposed index employs neural networks to learn %from query-object ground-truth relevant pairs, 
to cluster relevant geo-textual objects together while separating the irrelevant ones, and routes embedding based spatial keyword queries to relevant clusters through the neural networks to accelerate the top-k search process. %generate candidates, 
%our proposed index learns from query-object pairs in a data-driven manner and employs neural networks for data partitioning and query routing. 
Notably, our proposed index utilizes a novel learning-to-cluster technique to group embedding based geo-textual objects, while the IVF index employs the conventional $k$-means algorithm to cluster embeddings.


